Configuration-dependent Fault Localization

In a buggy configurable system, configuration-dependent bugs cause the failures in only certain configurations due to unexpected interactions among features. Manually localizing configuration-dependent faults in configurable systems could be highly time-consuming due to their complexity. However, the cause of configuration-dependent bugs is not considered by existing automated fault localization techniques, which are designed to localize bugs in non-configurable code. Thus, their capacity for efficient configuration-dependent localization is limited. In this work, we propose CoFL, a novel approach to localize configuration-dependent bugs by identifying and analyzing suspicious feature interactions that potentially cause the failures in buggy configurable systems. We evaluated the efficiency of CoFL in fault localization of artificial configuration-dependent faults in a highly-configurable system. We found that CoFL significantly improves the baseline spectrum-based approaches. With CoFL, on average, the correctness in ranking the buggy statements increases more than 7 times, and the search space is significantly narrowed down, about 15 times.

==> abstract.tex <==
\begin{abstract}
In a configurable system, configuration-dependent faults
cause the failures in only certain configurations because of feature
interactions. Manually localizing them in a configurable system
could be time-consuming due to its complexity. Meanwhile, exiting
automated fault localization techniques focus on localizing bugs in
particular buggy configurations.

In this work, we propose {\tool}, a novel approach to localize
configuration-dependent bugs in configurable systems. The inputs of
our algorithm include a buggy configurable system, the set of its
tested configurations including passed configurations and the
configurations that are failed at least one test, and the execution
information collected during the testing phase. {\tool} first
identifies the set of suspicious features whose combination reveals the
failure in all failed configurations, and their switching makes the
resulting configuration pass all the tests. Those suspicious features
are statically analyzed to detect the suspicious interactions between
them through program operations on the shared data structures/program
entities. These suspicious interactions are used to identify the
suspicious statements that are the executed statements having
dependency impact on the interactions. Finally, the suspicious
statements are ranked according to suspiciousness assessed using a
spectrum-based method.

We evaluated the effectiveness of {\tool} in fault localizing
artificial seeded configuration-dependent faults in a
highly-configurable system. We found that {\tool} significantly
improves the baseline spectrum-based approach. With {\tool}, on
average, the correctness in ranking the buggy statements increases
more than 9 times, and the search space is significantly narrowed
down, about 15 times.

\end{abstract}


==> alg_1.5.tex <==
\begin{algorithm}[t]
\caption{Suspicious Partial Configuration Detection}	
 \label{alg_1_5}
\begin{algorithmic}[1]
\Procedure {DetectSPCs}{$CP$, $CF$}
	\State $SPCList = EmptySet$
	\ForAll {$c \in CF$}
		\State $\wp = EmptySet$
		\ForAll {$c' \in CP$}
			\State $S = c \backslash (c' \cap c)$
			\If {$S \neq \emptyset$}
				\State $\wp.add(S)$
			\EndIf
		\EndFor
		\State $minimize(\wp)$
		\State $\partial = \bigcup_{\substack{S \in \wp}} S$
		\ForAll {$spc \in Subset(\partial)$}
			\If {$Satisfy(spc, CP, CF)$}
				\State $SPCList.add(S)$
			\EndIf
		\EndFor
	\EndFor
	\State $minimize(SPCList)$
\EndProcedure
\Statex

\end{algorithmic}
\end{algorithm}


==> alg_1.tex <==
\begin{algorithm}
\caption{{\tool}: Single suspicious partial configuration detection algorithm}	
 \label{alg_1}
\begin{algorithmic}[1]
\Procedure {DetectSPC}{$c$, $CP$}
\State $SPC = EmptySet$

\ForAll {$s \in c$}
	\State $subset = c.subtract(s)$
	\ForAll {$PassingConfig \in CP$}
		\If {$PassingConfig.containsAll(subset)$}
			\State $SPC.adds(s)$
			\State $break$
		\EndIf
	\EndFor
\EndFor
\EndProcedure
\Statex

%OLD
%\Procedure {DetectSPC}{$CP$, $CF$}
%\State $SPC = EmptySet$
%\State $examinedSels = commonSubSet(CF)$
%
%\ForAll {$s \in examinedSels$}
%	\State $subset = examinedSels.subtract(s)$
%	\ForAll {$passedConfig \in CP$}
%		\If {$passedConfig.containsAll(subset)$}
%			\State $SPC.add(s)$
%			\State $break$
%		\EndIf
%	\EndFor
%\EndFor
%\EndProcedure
%\Statex

%\Procedure {FindUnrelatedFeatures}{$CF$}
%\State $unrelatedFeatures = EmptySet$
%
%\ForAll {$f \in AllFeatures$}
%	\State $enabledSel = enable(f)$
%	\State $disabledSel = disable(f)$
%	\State $config = findContainingConfig(enabledSel, CF)$
%	\State $other = findContainingConfig(disabledSel, CF)$
%	\If {$config \neq NULL \wedge other \neq NULL$ }
%		\State $addToSet(f, unrelatedFeatures)$
%	\EndIf
%\EndFor
%\EndProcedure
%\Statex
\end{algorithmic}
\end{algorithm}


==> alg_2.tex <==
\begin{algorithm}
\caption{{\tool}: Feature interaction detection}	
 \label{alg_2}
\begin{algorithmic}[1]
\Procedure {DetectInteractionImpl}{$f_1$, $f_2$}
\State $InteractionImpl = EmptySet$
\State $DD = def(f_1) \cap def(f_2)$
\State $DU = def(f_1) \cap use(f_2)$
\State $UD = use(f_1) \cap def(f_2)$
\ForAll {$e \in DD$}
	\State $defStmsF1 = def(f_1) \cap Define(e)$
	\State $InteractionImpl.adds(defStmsF1)$
	\State $defStmsF2 = def(f_2) \cap  Define(e)$
	\State $InteractionImpl.adds(defStmsF2)$
\EndFor
\ForAll {$e \in DU$}
	\State $defStmsF1 = def(f_1) \cap Define(e)$
	\State $InteractionImpl.adds(defStmsF1)$
	\State $useStmsF2 = use(f_2) \cap Use(e)$
	\State $InteractionImpl.adds(useStmsF2)$
\EndFor
\ForAll {$e \in UD$}
	\State $useStmsF1 = use(f_1) \cap Use(e)$
	\State $InteractionImpl.adds(useStmsF1)$
	\State $defStmsF2 = def(f_2) \cap Define(e)$
	\State $InteractionImpl.adds(defStmsF2)$
\EndFor
\EndProcedure
\Statex
\end{algorithmic}
\end{algorithm}



%\begin{algorithm}
%\caption{{\tool}: Feature interaction detection}	
% \label{alg_2}
%\begin{algorithmic}[1]
%\Procedure {DetectInteractionImplementation}{$F1$, $F2$}
%\State $InteractionImpl = EmptySet$
%\State $DD = intersection(def(F1), def(F2))$
%\State $DU = intersection(def(F1), use(F2))$
%\State $UD = intersection(use(F1), def(F2))$
%\ForAll {$e \in DD$}
%	\State $def1 = intersection(def(F1), Define(e))$
%	\State $InteractionImpl.add(def1)$
%	\State $def2 = intersection(def(F2), Define(e))$
%	\State $InteractionImpl.add(def2)$
%\EndFor
%\ForAll {$e \in DU$}
%	\State $def1 = intersection(def(F1), Define(e))$
%	\State $InteractionImpl.add(def1)$
%	\State $use2 = intersection(use(F2), Use(e))$
%	\State $InteractionImpl.add(use2)$
%\EndFor
%\ForAll {$e \in UD$}
%	\State $use1 = intersection(use(F1), Use(e))$
%	\State $InteractionImpl.add(use1)$
%	\State $def2 = intersection(def(F2), Define(e))$
%	\State $InteractionImpl.add(def2)$
%\EndFor
%\EndProcedure
%\Statex
%\end{algorithmic}
%\end{algorithm}

==> alg_3.tex <==
\begin{algorithm}
\caption{{\tool}: Suspicious statement detection}	
 \label{alg_3}
\begin{algorithmic}[1]
\Procedure {DetectSuspiciousStatement}{$code$, $CP$, $CF$, $testresults$, $executionInfo$}
\State $SuspiciousStatements = EmptySet$
\ForAll {$c \in CF$}
	\State $SPC = DetectSPC(c, CP)$
	\State $EnabledFeatures = GetEnabledFeatures(SPC)$
	\State $DisabledFeatures = GetDisabledFeatures(SPC)$
	\ForAll {$f1, f2 \in EnabledFeatures$, $f1 \neq f2$}
		\State $impl = DetectInteractionImplementation(f1, f2)$
		\State $impl = RemoveUnrelatedStms(impl, DisabledFeatures)$
		\State $SuspiciousStatements.adds(impl)$
	\EndFor	
\EndFor
\State $SpectrumBasedRank(SuspiciousStatements, executionInfo)$
\EndProcedure
\Statex
\end{algorithmic}
\end{algorithm}

==> algorithm.tex <==
\section{Configuration-dependent Fault Localization}
\subsection{Overview}
The input for our configuration-dependent fault localization algorithm 
includes the buggy configurable system, the test results of each 
configurations and the executed statements that are recorded for each 
tests in each configuration. 
In general, to localize a configuration-dependent bug, our algorithm
works in three following steps.

1) It first identifies the feature selection candidates for the
fault-causing partial configuration for the bug. The resulting set of
feature selections is called the \textit{suspicious partial
  configuration} that potentially causes the bug.

2) Next, the features in the suspicious partial configuration, whose
interactions between them are most likely to cause the
configuration-dependent bug, are analyzed to detect the statements
that implement those interactions.

3) Finally, these suspicious statements are used to 
detect other suspicious statements that are executed and have 
impact on them in the failed configurations.
%


==> concept.tex <==
\section{•}

==> concepts.tex <==
\section{Concepts and Problem Statement}
\label{concepts_section}

In a configurable system, a \textit{feature} is an optional
functionality in addition to a special feature - \textit{the core
  feature} (i.e., \textit{the base variant}) which is enabled in every variant of the system. Features
are implemented as statically conditional statements\footnote{For the
  purpose of localization, we assume that statement is the unit of
  program that need to be considered in the fault localization
  problem.} guarded by constraints over feature symbols (e.g.,
\texttt{\#if} macro). In Figure~\ref{example_bug}, feature \texttt{LOCKDEP}
contains the set of statements from line 20 to 27.

%Feature
\begin{definition}{({\bf Feature}).}
A feature is implemented as a set of optional statements that are 
guarded by constraints over feature symbols. Given a configurable 
system implemented by a set of statements $\mathbb{S}$, we define a function 
$\varphi: \mathbb{F}\to 2^{\mathbb{S}}$, where $\mathbb{F}$ is the set of features in the 
configurable system. $\varphi(f)$ refers to the set of statements 
that implement feature $f$.
\end{definition}



In Figure~\ref{example_bug}, $\varphi($\texttt{SLAB}$)$ is the set of
statements from lines 11--12, while
$\varphi($\texttt{PPC\_256K\_PAGES}$)$ contains only line 4.

\begin{definition}{({\bf Feature Selection}).}
A feature selection of feature $f$ is a state of the feature that is 
either enabled or disabled ($f=T/F$ for short).
\end{definition}
%
In preprocessor-based program families \cite{kastner2012virtual}, a 
feature selection is controlled by one or more \textit{configuration 
options} (macro symbols). In the example, the feature \texttt{LOCKDEP} 
is controlled by the configuration option \texttt{CONFIG\_LOCKDEP}.
%
In a configurable system, the selections of features are used to specify
particular configurations (variants) of the system.
%

%Configuration
\begin{definition}{({\bf Configuration}).}
In a configurable system consisting of the set of features
$\mathbb{F}$, a configuration $c$ is a particular set of the
selections for all features in $\mathbb{F}$. 
\end{definition}

For fault localization, it is often that we do not have
test cases for all feasible configurations of the system. In practice,
we might have only a subset of configurations with corresponding test
cases.

\begin{definition}{({\bf Available Configurations}).}
  The set $\mathbb{C}$ of given configurations with executed test
  results are called available configurations.
%  We denote $\mathbb{C}$ as the set of all available executed configurations of the system.
\end{definition}

%In practice, a 
%configuration-dependent bug can be revealed during testing process, when 
%there are configurations failing at least one test, while others pass 
%all their test cases. Even after the system have been released, many 
%configuration-dependent bugs are newly reported by the end-users when they execute the configurations in their own environments.
%

In practice, a {\em configuration-dependent} bug can be revealed
during testing, in which there are configurations failing at least
one test, while others pass all their tests.
% Moved to intro
%Even after the system have been released, many configuration-dependent
%bugs are newly reported by the end-users when they execute the
%configurations in their own environments.
%
%For example, the bug in Fig.~\ref{example_bug} is revealed only in
%$c_2$ and $c_7$ in which the features \texttt{LOCKDEP},
%\texttt{PPC\_256K\_PAGES}, \texttt{\!SLOB}, and \texttt{SLAB} are all
%enabled and \texttt{PPC\_16K\_PAGES} is disabled.
%
%
For example, the bug in Figure~\ref{example_bug} is revealed only in
$c_2$ and $c_7$ in which the features \texttt{LOCKDEP},
\texttt{PPC\_256K\_PAGES}, \texttt{!SLOB}, and \texttt{SLAB} are
enabled and \texttt{PPC\_16K\_PAGES} is disabled.
%
In highly configurable systems, most of reported bugs  are 
configuration-dependent faults that are only exposed under a set of 
certain configurations \cite{Abal:2018} \cite{Garvin:2011}. 

%

\begin{definition}{({\bf Configuration-dependent Fault}).}
In a configurable system, a fault is considered as a
configuration-dependent bug if only if there are two non-overlapping
partitions of configurations $CP$ and $CF$, where $CP, CF \subsetneq
\mathbb{C}$, $CF \cup CP = \mathbb{C}$, and $CF \cap CP = \emptyset$,
such that all configurations in $CP$ execute as expected, while each
of the configurations in $CF$ has at least one failed test.
%reveal the bug.
\end{definition}

In Table~\ref{test_results},  $\mathbb{C}=\{c_1, ..., c_7\}$, and $CF=\{c_2, c_7\}$, $CP=\{c_1, c_3, c_4, c_5, c_6\}$.

\begin{definition}{({\bf Configuration-dependent Fault Localization}).}
Given buggy configurable code, the test result of each configuration
in the available configuration set $\mathbb{C}$, and the trace of the
executed statements that are recorded for each test in each
configuration, configuration-dependent fault localization is to output
the ranked list of statement(s) that are likely to cause the fault(s).
\end{definition}


==> conclusion.tex <==
\section{Conclusion}

In this work, we propose {\tool}, a novel approach to localize
configuration-dependent bugs in configurable systems. The inputs of
our algorithm include a buggy configurable system, the set of its
tested configurations including passed configurations and the
configurations that are failed at least one test, and the execution
information collected during the testing phase. {\tool} first
identifies the set of suspicious features whose combination reveals the
failure in all failed configurations, and their switching makes the
resulting configuration pass all the tests. Those suspicious features
are statically analyzed to detect the suspicious interactions between
them through program operations on the shared data structures/program
entities. These suspicious interactions are used to identify the
suspicious statements that are the executed statements having
dependency impact on the interactions. Finally, the suspicious
statements are ranked according to suspiciousness assessed using a
spectrum-based method. We evaluated the effectiveness of {\tool} in
fault localizing artificial seeded configuration-dependent faults in a
highly-configurable system. We found that {\tool} significantly
improves the baseline spectrum-based approach. With {\tool}, on
average, the correctness in ranking the buggy statements increases
more than 9 times, and the search space is significantly narrowed
down about 15 times.


==> discussion.tex <==
\section{Discussion}


==> eval.tex <==
\section{Empirical Evaluation}
To evaluate {\tool}, we answer the following questions:
\begin{itemize}
%\item \textbf{RQ1 [Comparison]}: How does {\tool} improve Tarantula when we 
%run {\tool} with the spectrum-based method? 
\item \textbf{RQ1 [Comparison]}: How does {\tool} improve a spectrum-based 
approaches when we run {\tool} with these methods? 
\item \textbf{RQ2 [Time Complexity]}: What is {\tool}'s running time?
\end{itemize}
\subsection{Subject system}
In this work, we seeded 32 configuration-dependent bugs into 
BusyBox~\cite{busybox} as the subject system which is a highly-configurable 
system containing about 190KLOC in about 800 files and more than 1,400 
configuration options. We selected \textbf{100} configurations to test and 
collected execution information for localizing these bugs. 
\subsection{Comparison and Effectiveness (RQ1)}

\input{experimental_procedure}

\subsubsection{Metric}
For evaluation, we use $EXAM$ \cite{exam}, a widely-used metric in evaluating 
fault localization techniques. $EXAM$ is the portion of statements in a program 
that has to be examined until the first faulty statement is reached:
%
$$EXAM = \frac{N}{T} \times 100\%$$ 
%
where $N$ is the number of statements examined, and $T$ is the total number of 
statements in the program. The lower $EXAM$, the more effective the bug 
localization technique.

\subsubsection{Results}

\input{results_tb}

Table \ref{results_tb} shows the the comparative results between the average 
$EXAM$, average rank, and average search space size of {\tool} and the baseline 
fault localization method, when we ran them on set of artificial configuration-
dependent bugs.

As seen, {\tool} achieves about 32\% lower $EXAM$ than Tarantula and Ochiai. The 
correctness in ranking the faulty statements is also improved by more than 
\textbf{9} times over the spectrum-based methods when we ran {\tool} with them.
%By {\tool}, the search space for the buggy statements is also significantly narrowed down (about \textbf{Z} times). 
On average, a developer has to inspect only \textbf{single} statement by
using {\tool} with Tarantula compared to \textbf{9} statements by
using only a spectrum-based technique. The reason of this
phenomenon is that Tarantula assigns exactly the same suspiciousness
score to the statements that have the same execution pattern (e.g.,
the same \texttt{if} branch). Therefore, all statements implementing
the same feature, even the statements that have no impact on other
features or the state of the program (e.g, \texttt{printf()} statement)
might be assigned the same suspiciousness level. This is also a
general weakness of the spectrum-based fault localization methods
\cite{wong2009survey}. This weakness is also reflected by the
results shown in Table~\ref{results_tb} that the differences between the
performance of these spectrum-based techniques are not significant,
only about 1.0\% ($EXAM$~score).

\begin{figure}[h]
\begin{center}
\lstinputlisting[captionpos=b]{example_4.c}
\caption{A configuration-dependent bug seeded into BusyBox}
\label{bug_result}
\end{center}
\end{figure}

Fig. \ref{bug_result} shows an example of a configuration-dependent
bug seeded into BusyBox. The bug is revealed only in the configuration
which enables both \texttt{FEATURE\_HTTPD\_RANGES} and
\texttt{FEATURE\_USE \_SENDFILE}, and disables
\texttt{FEATURE\_HTTPD\_GZIP}. In this configuration,
\texttt{range\_start} is assigned an incorrect value, \texttt{0}, at
line 20 instead of \texttt{-1} as expected at at line 19. The
incorrect value of \texttt{range\_start} is propagated to
\texttt{FEATURE \_USE\_SENDFILE} where the variable is used at lines
26 and 31. However, this failure is not observed when
\texttt{FEATURE\_HTTPD\_GZIP} is on. In this case,
\texttt{content\_gzip} is defined as 0 at line 11. That makes the
statement at line 20 never being executed. For this bug, after the $SPC$,
$\{$\texttt{FEATURE\_HTTPD\_RANGES = T},
\texttt{FEATURE\_USE\_SENDFILE = T}, \texttt{FEATURE\_HTTPD\_GZIP =
  F}$\}$ is detected, the configurable code is analyzed to detect the
statements that implement the interactions between
\texttt{FEATURE\_USE\_SENDFILE} and \texttt{FEATURE\_HTTPD\_RANGES}
(lines 20, 21, 26, 31 and 32). The statements that have certain
dependency impact on the implementation might be suspicious. However,
if they do not have any dependency relation with statements at line 11
and 18 that implement the interaction between
\texttt{FEATURE\_HTTPD\_GZIP} and \texttt{FEATURE\_HTTPD\_RANGES},
they are not affected by \texttt{FEATURE \_HTTPD\_GZIP} and execute as
expected when the feature is enabled.  Consequently, they are not
considered to be faulty. As results, the set of suspicious statements
detected by {\tool} includes the executed statements at lines 18, 20, 26
and 31.

\begin{figure}[h]
\begin{center}
\lstinputlisting[captionpos=b]{example_5.c}
\caption{An example that {\tool} did not detect well the buggy statement}
\label{bug_limit}
\end{center}
\end{figure}

Fig. \ref{bug_limit} shows an example that {\tool} did not localize
well the faulty statement at line 12. The bug is revealed when
\texttt{FEATURE\_LS\_FILETYPES} and \texttt{FEATURE\_LS\_USERNAME} are
both enabled. By {\tool}, several non-buggy statements are considered
as suspicious statements. First, the statements at lines 10 and 21
that define \texttt{column} shared by \texttt{FEATURE\_LS\_FILETYPES}
and \texttt{FEATURE\_LS\_USERNAME} are considered to be suspicious by
{\tool}. However, if the buggy statement were one of them, the fault
would have been revealed when one of these features is enabled instead
of both of these features. Indeed, for example, if statement at line
10 is faulty, whenever \texttt{FEATURE\_LS\_USERNAME} is on,
\texttt{display\_single} will return an unexpected output.
Additionally, the statements at line 9 that use \texttt{opt} in
\texttt{FEATURE\_LS\_USERNAME} and line 22 in
\texttt{FEATURE\_LS\_FILETYPES} that defines the entity are also
considered to be suspicious by {\tool}. Still, since the statement at
line 9 is executed before the one at line 22 in the function, these
statements do not affect each other.

The reason for both situations is that {\tool} detects the interaction
between features by pairs of them without considering the order of the
features in each pair. We design {\tool} to detect the interaction
between features by pairs in order to improve the scalability and
applicability to localize bug in large-scale configurable systems that
are usually highly complex. We do not consider the order factor of
features for the following reasons. First, for a pair of features,
they might include several optional blocks of code, however the
execution order of the blocks in two features might be
inconsistent. This makes the execution order of the features
undecidable. Additionally, the order of the use and definition of a
global variable in different functions defined by features might be
undecidable without considering these functions in a particular
function where they are called.
%

\subsection{Time Complexity (RQ2)}
%Analyze 399095
%
We run our experiments on a desktop computer with Intel Core i5 2.7GHz processor, 
8GB RAM. Table \ref{running_time} shows the average running time of {\tool} to 
analyze a large scale configurable system with 190KLOC and more than 1,400 
configuration options and detect configuration-dependent bugs that  are caused by 
the interaction between 2 to 7 features. Note that all reported configuration-
dependent bugs require developers to enable or disable up to seven features.
%
As seen, on average, {\tool} can analyze and localize almost configuration-
dependent bugs in the subject system in around 408s. Moreover, the running time 
of {\tool} is insignificantly increased by the increment of the number of 
features related to the faults. The reason of this phenomenon is that {\tool} 
analyzes and detects the interactions between features by pairs of features, 
which leads to the scalability of {\tool} by the size of feature interactions.

\begin{table}[]
\small
\centering
\caption{The running time of {\tool} by bug's feature interaction levels}
\label{running_time}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
Level & 2 & 3 & 4\\ \hline
Time (ms) & 399,115 &400,110 & 402,242 \\ \hline
\rowcolor[HTML]{C0C0C0} 
Level & 5 & 6 & 7\\ \hline
Time (ms) & 403,385 & 405,450 & 408,120 \\ \hline
\end{tabular}
\end{table}


==> experimental_procedure.tex <==
\subsubsection{Experimental Procedure}
Since constructing a database of real configuration-dependent bug and the tests of the corresponding system is a considerable task, until now there is no public database for configuration-dependent bug that contains the tests of the corresponding configurable system. Thus, in this paper, to evaluate in the ability of {\tool} in localizing configuration-dependent bugs, we first seeded artificial configuration-dependent bugs into a particular configurable system~\cite{mutation1, mutation2, mutation3}. 
%
To seed a single configuration-dependent into the subject system, we randomly performed a single mutation operation: \textit{add} or \textit{update} a statement, that follows the guideline in \cite{Garvin:2011}. Especially, the mutant system must be satisfied both following conditions:
\begin{enumerate}
\item There exists at least one configuration that fails at least one of its tests.
\item There exists at least one variant of the system that passes all of its tests.
\end{enumerate}
%
Those bugs can be found in our website \cite{website}. After that, for each buggy version of the configurable system that
contains a single bug, we selected a set of configurations for testing
\cite{sampling}. Then, these configurations were tested separately to
collect the execution information. For comparison, we ran {\tool} with
the spectrum-based techniques on the system and the collected
execution information to see the improvement of {\tool} over these
spectrum-based techniques.

The reason for such choice of the baseline model is that a
spectrum-based fault localization technique does not work effectively
for a configurable code because it is not designed for configurable
code as explained earlier. However, by combining with {\tool}, the
suspicious statements are identified by {\tool}, and a spectrum-based
fault localization technique now can effectively work on the
configurable code to assign the correct suspiciousness scores.

==> expriment_produce.tex <==
\subsubsection{Experimental Procedure}
Since constructing a database of real configuration-dependent bug and the tests of the corresponding system is a considerable task, until now there is no public database for configuration-dependent bug that contains the tests of the correspoinding configurable system. Thus, in this paper, to evaluate in the ability of {\tool} in localizing configuration-dependent bugs, we first seeded artificial configuration-dependent bugs into a particular configurable system~\cite{mutation1, mutation2, mutation3}. 
%
To seed a single configuration-dependent into the subject system, we randomly performed a single mutation operation: \textit{add} or \textit{update} a statement, that follows the guideline in \cite{Garvin:2011}. Especially, the mutant system must be satisfied both following conditions:
\begin{enumerate}
\item There exists at least one configuration that fails at least one of its tests.
\item There exists at least one variant of the system that passes all of its tests.
\end{enumerate}
%
Those bugs can be find in our website \cite{website}. After that, for each buggy version of the configurable system that
contains a single bug, we selected a set of configurations for testing
\cite{sampling}. Then, these configurations were tested separately to
collect the execution information. For comparison, we ran {\tool} with
the spectrum-based techniques on the system and the collected
execution information to see the improvement of {\tool} over these
spectrum-based techniques.

The reason for such choice of the baseline model is that a
spectrum-based fault localization technique does not work effectively
for a configurable code because it is not designed for configurable
code as explained earlier. However, by combining with {\tool}, the
suspicious statements are identified by {\tool}, and a spectrum-based
fault localization technique now can effectively work on the
configurable code to assign the correct suspiciousness scores.

==> feature_interaction_algo.tex <==
\subsection{Feature interaction detection}

For each $SPC$, {\tool} analyzes each feature whose selection is in the $SPC$ to detect the statements used to implement the interactions among those features. For each pair of features, $f_1$ and $f_2$, we use Algorithm~\ref{alg_2} to detect the interaction between them. First, the algorithm identifies shared program entities between $f_1$ and $f_2$, which might be (re-)defined by the two features or defined by a feature and used by
other (lines 3--5). After that, those shared entities are used to detect the set of statements ($InteractionImpl$) that implement their definitions (lines 6--10) and the definitions and uses of those entities (lines 11--20) in the two features.

\input{alg_2}

For example, by Algorithm~\ref{alg_2}, the set of statements that 
implement the interaction between \texttt{!SLOB} and 
\texttt{LOCKDEP} through \texttt{kmalloc} \texttt{\-\_caches} contains the 
statements at line 16 (\texttt{kmalloc\_caches} is defined) and 
at line 24 (the entity is used).


==> feature_interaction_formulation.tex <==
\subsection{Formulation}
%Entity
\begin{definition}{({\bf Program Entity}).}
A program entity is a program element uniquely identified with
a \textit{name} and a \textit{scope}.
\end{definition}

In our formulation, we are interested in two types of program
entities: {\em variable} and {\em function}.
%
An entity is represented in the form of \texttt{[scope.ent\_name]},
where \texttt{scope} and \texttt{ent\_name} are the scope and the 
name of the program entity respectively. The \textit{scope} and the
\textit{name} of an entity are used together as the identity of the
entity. For example, the code in Fig.~\ref{example_bug} contains
variables \texttt{GLOBAL.kmalloc\_caches}, \texttt{init\_node
\_lock\_keys.i}, and function \texttt{GLOBAL.init\_lock\_keys}.
%

%Program Operation
In our work, there are two {\bf program operations} on variables and
functions: \textit{define (def)} and \textit{use}. A \textit{def}
operation is used to \textit{assign} a value to a variable or
\textit{define} the body for a function. Meanwhile, a variable is
\textit{used} when it is \textit{used} or \textit{referred} to. A
function is \textit{used} if it is \textit{called}/\textit{invoked} or
used as a function pointer (C/C++). For example, the function
\texttt{GLOBAL.init\_node\_lock\_keys} is \textit{defined} as a set of
statements from lines 21--26 and \textit{called/used} at line 33. For variable \texttt{X}, it might be \textit{declared}
or \textit{destructed}. However, without loss of generality, when
\texttt{X} is declared or destructed, we consider that it is
\textit{defined} with \texttt{UNINIT} or \texttt{UNDEFINED}
respectively. For instance, the value of
\texttt{init\_node\_lock\_keys.i} is \texttt{UNINIT} at line 21.
%
%Implementation Functions

Given a program, $E$ is the set of program entities, and $\mathbb{S}$
is the set of statements of the program, we use 2
\textit{implementation functions} to map each entity in $E$ to the
sets of statements in $\mathbb{S}$ that implement its definitions and
uses:
\begin{definition}{({\bf Implementation Functions}).}
\begin{itemize}
  \item $Define:E \to 2^\mathbb{S}$, $Define(e)$ is the set of statements that 
  implement the {\bf definitions} of $e$
  \item $Use:E \to 2^\mathbb{S}$, $Use(e)$ is the set of statements that 
  implement the {\bf uses} of $e$
\end{itemize}
\end{definition}
In Fig.~\ref{example_bug},
$Define($\texttt{GLOBAL.kmalloc\_caches}$)$ contains only statements
at line 16, while, the statement at line 24 is the only element of
$Use($\texttt{GLOBAL.kmalloc\_caches}$)$. For compound
statements, we also consider the conditional expressions
(\textit{if-statement}, \textit{for-loop}, \textit{while-loop} and
\textit{do-loop}), the control expressions or the options
(\textit{switch-statement}), and take them into account for localizing
bugs.

%Feature
\begin{definition}{({\bf Feature-related Functions}).}
In a configurable system, which is implemented by a set of statements 
$S$ and consists of a set of features $F$ and a set of program 
entities $E$, we define two feature-related functions:
\begin{itemize}
	\item $def:F \to 2^E$, $\forall e \in E, e \in def(f) 
	  \Leftrightarrow 	Define(e) $ $\cap \quad \varphi(f) \neq \emptyset$. That is, if the set of statements implementing the definitions of $e$ overlaps with the set of statements realizing the feature $f$, then $e$ belongs to $def(f)$.
          For a program entity, $def(f)$ is the set of program entities which are defined within 
	$f$, e.g., \texttt{cpuup\_prepare.node} $\in def($\texttt{NUMA}$)$.
	%	
	For a function, $f$ is used to realize their definition. For instance, since the statement at line 31 in \texttt{NUMA} is used to define the body of \texttt{GLOBAL.cpuup\_prepare}, this entity is also an element of $def($\texttt{NUMA}$)$.

	\item $use:F \to 2^E$, $\forall e \in E, e \in use(f)
          \Leftrightarrow Use(e) $ $\cap \quad \varphi(f) \neq
          \emptyset$.  That is, if the set of statements~implementing
          the uses of $e$ overlaps with the set of statements realizing the feature $f$, then $e$ belongs to $use(f)$.
          %
	Specifically, $use(f)$ is the set of program entities~that are used within $f$, 
	e.g., \texttt{GLOBAL.PAGE\_SHIFT}, \texttt{GLOBAL.kmalloc\_cach\-es},~\texttt{GLOBAL.slab\_set\_lock\_classes} $\in use($\texttt{LOCKDEP}$)$.
	
\end{itemize}
\end{definition}

In a configurable system, two features can interfere each other 
through the program entities that are shared to implement these 
features, or they can interact via the dependency affection between 
their entities. In the running example, \texttt{LOCKDEP} \textit{uses} 
\texttt{PAGE\_SHIFT} (line 22) and \texttt{kmalloc\_caches} (line 24) 
that are \textit{defined} by \texttt{SLAB} (line 11) and 
\texttt{!SLOB} (line 16) respectively to implement its functionality.
Hence, the optional functionality offered by \texttt{LOCKDEP} is
influenced when \texttt{SLAB} or \texttt{!SLOB} are enabled/disabled.
%
%
In this work, we focus on the feature interactions through program entities. The interactions associated with external data such 
as files or database are beyond the scope of this work. By that our assumption,, if both 
features \textit{use} a program entity, they will not change the 
program's state. Therefore, there is no interaction 
between two or more features if they only \textit{use} the same 
program entities. 

%
%Feature Interaction
\begin{definition}{({\bf Feature Interaction}).}
The interaction between two features $f_1$ and $f_2$ exists if only if:
\begin{itemize}
	\item $def(f_1) \cap def(f_2) \neq \emptyset$
	\item $def(f_1) \cap use(f_2) \neq \emptyset$ or $def(f_2) \cap use(f_1) \neq \emptyset$
	\item $\exists e_1 \in def(f_1), e_2 \in use(f_2)$, such that
	$e_2 \in affection(e_1, c)$, or $e_1 \in affection(e_2, c)$, where function $affection(e, c)$ specifies 
	the set of program entities that are affected by $e$ in the particular configuration, $c$. In the running example, \texttt{cache} $\in affection($\texttt{MAX\_ORDER}$, c_1)$
\end{itemize}
\end{definition}
%

By the above definition, we only represent the interaction between a 
pair of features because the interaction between more than two 
features is still represented by the interactions of pairs features. 
Indeed, assuming that there exists an interaction among $m > 2$ 
features. For simplicity, we consider the case of m = 3, $f_1$, 
$f_2$, and $f_3$, and $E_1$, $E_2$, and $E_3$ are the sets of share 
program entities of three pairs of features ($f_1$, $f_2$), ($f_2$, $f_3$), and ($f_3$, $f_1$).
%
If there exists a common entity shared between all these features, 
the interaction among them is still represented through the interactions 
of the pairs.
%
On the other case, there is no shared entity between all features, 
assuming that $E_1 \cap E_3 = \emptyset$. Since the functionality 
offered by $f_3$ is influenced by $f_1$\footnote{because the roles of 
$f_1$ and $f_3$ in this case are equal} through $f_2$, there exists 
an entity $e_1 \in def(f_1)$ whose value affects another entity $e_3 
\in use(f_3)$ by a value propagation function $p$, such that $e_3 = 
p(e_1)$. Hence, by identifying feature interactions between pairs, 
the interactions among more than two features are still captured. 
%
%
%\begin{definition}{({\bf Feature Interaction Implementation}).} The implementation of the interaction between features $f_1$ and $f_2$ are the statements that implement the definitions of the shared entities in $f_1$ and $f_2$ (for def-def interactions) and the uses of the shared entities in $f_1$ and $f_2$ (for def-use interactions).
%\end{definition}



==> formulation.tex <==
\section{Formulation}
In this section, we provide our formulation of the problem of
configuration-dependent fault localization.
%
%
%Entity
In a program, we are interested in the program entities and the
operations that are performed on them.
\begin{definition}{({\bf Program Entity}).}
A program entity is a program element uniquely identified with
a \textit{name} and a \textit{scope}.
\end{definition}

In our formulation, we are interested in two types of program
entities: {\em variable} and {\em function}.
%
An entity is represented in the form of \texttt{[scope.ent\_name]},
where \texttt{scope} and \texttt{ent\_name} are the scope and the 
name of the program entity respectively. The \textit{scope} and the
\textit{name} of an entity are used together as the identity of the
entity. For example, the code in Fig.~\ref{example_bug} contains
variables \texttt{GLOBAL.kmalloc\_caches}, \texttt{init\_node
\_lock\_keys.i}, and function \texttt{GLOBAL.init\_lock\_keys}.
%

%Program Operation
In our work, there are two program operations on variables and
functions: \textit{define (def)} and \textit{use}. A \textit{def}
operation is used to \textit{assign} a value to a variable or
\textit{define} the body for a function. Meanwhile, a variable is
\textit{used} when it is \textit{used} or \textit{referred} to. A
function is \textit{used} if it is \textit{called}/\textit{invoked} or
used as a function pointer (C/C++). For example, the function
\texttt{GLOBAL.init\_node\_lock\_keys} is \textit{defined} as a set of
statements from lines 21--26 and \textit{called/used} in the statement
at line 33. For a variable \texttt{X}, it might be \textit{declared}
or \textit{destructed}. However, without loss of generality, when
\texttt{X} is declared or destructed, we consider that it is
\textit{defined} with \texttt{UNINIT} or \texttt{UNDEFINED} respectively. For instance, the value of
\texttt{init\_node\_lock\_keys.i} is \texttt{UNDEFINED} at line 21.
%

%Implementation Functions
Given a program, we define 2 \textit{implementation functions} as 
the functions from $E$ to $2^S$, where $E$ is the set of program 
entities, and $S$ is the set of statements of the program:
\begin{definition}{({\bf Implementation Functions}).}
\begin{itemize}[leftmargin=4mm]
  \item $Defined:E \to 2^S$, $Defined(e)$ is the set of statements that 
  implement the {\bf definitions} of $e$
  \item $Used:E \to 2^S$, $Used(e)$ is the set of statements that 
  implement the {\bf uses} of $e$
\end{itemize}
\end{definition}
In Fig.~\ref{example_bug},
$Defined($\texttt{GLOBAL.kmalloc\_caches}$)$ contains only statements
at line 16, while, the statement at line 24 is the only element of
$Used($\texttt{GLOBAL.kmalloc\_caches}$)$. For the compound
statements, we also consider the conditional expressions (\textit{if-statement}, \textit{for-loop}, \textit{while-loop} and \textit{do-loop}), the control expressions or the options (\textit{switch-statement}) and take them into account for localizing bugs.
%
% Break flow

%

%
%In practice, a feature (parent-feature) might contain several other features 
%(child-features). For example,...

%Feature
\begin{definition}{({\bf Feature-related Functions}).}
In a configurable system, which are implemented by a set of statements 
$S$ and consists of a set of features $F$ and a set of program 
entities $E$, we define two feature-related functions:
\begin{itemize}[leftmargin=4mm]
	\item $def:F \to 2^P$, $\forall e \in P, e \in def(f) 
	\Leftrightarrow 	Defined(e) $ $\cap \quad \varphi(f) \neq \emptyset$. 
	$def(f)$ is the set of program entities which are defined within 
	$f$, e.g., \texttt{cpuup\_prepare.node} $\in def($\texttt{NUMA}$)$; 
	%	
	or for functions, $f$ is used to realize their definition. For instance, since the statement at line 31 in \texttt{NUMA} is used to realize \texttt{GLOBAL.cpuup\_prepare}, this entity is also an element of $def($\texttt{NUMA}$)$.

	\item $use:F \to 2^E$, $\forall e \in P, e \in use(f)
	\Leftrightarrow Used(e) $ $\cap \quad \varphi(f) \neq \emptyset$. 
	$use(f)$ is the set of program entities that are used within $f$, 
	e.g., \texttt{GLOBAL.PAGE\_SHIFT}, \texttt{GLOBAL.kmalloc\_caches},~\texttt{GLOBAL.slab\_set\_lock\_classes} $\in use($\texttt{LOCKDEP}$)$.
	
%  \item $children: F \to 2^F$, $children(f)$ is the set of features that are 
%  child-features of $f$
%  \item $parent: F \to F$, $parent(f)$ the feature that $f$ is one of child-features of
\end{itemize}
\end{definition}
%
%
%\textit{The core feature}, $\Omega$, has no parent-feature, while every feature is
%contained by another one. If a (parent) feature is disabled, its child-features 
%are also disabled, and if one of child-features of a feature is enabled, the 
%feature is also enabled.

In a configurable system, two features can interfere each other 
through the program entities that are shared to implement these 
features. In the running example, \texttt{LOCKDEP} \textit{uses} 
\texttt{PAGE\_SHIFT} (line 22) and \texttt{kmalloc\_caches} (line 24) 
that are \textit{defined} by \texttt{SLAB} (line 11) and 
\texttt{!SLOB} (line 16) respectively to implement its functionality.
Hence, the optional functionality offered by \texttt{LOCKDEP} is
influenced when \texttt{SLAB} or \texttt{!SLOB} are enabled/disabled.
%
%
In this work, we focus on the feature interactions through shared 
program entities. The interactions associated with external data such 
as files or database are beyond the scope of this work. If both 
features \textit{use} a program entity, they will not change the 
program's state. By that our assumption, there is no interaction 
between two or more features if they only \textit{use} the same 
program entities. 
%The feature interaction between two features through 
%shared entities and $def$ and $use$ is described by the following 
%definition.

%
%Feature Interaction
\begin{definition}{({\bf Feature Interaction}).}
The interaction between two features $f_1$ and $f_2$ exists if only if 
$def(f_1) \cap def(f_2) \neq \emptyset$ (def-def) or $def(f_1) \cap use(f_2) \neq \emptyset$ (def-use). The statements that implement the definitions of the shared entities in $f_1$ and $f_2$ (def-def) and the uses of the share entities in $f_2$ (def-use) are the statements that implement the interactions.
\end{definition}
%
%$\bigcup_{e \in D} 
%(Defined(e) $ $\cap \varphi(f_1)) \cup \bigcup_{e \in D} (Defined(e) $ $
%\cap \varphi(f_2))$
%$\bigcup_{e \in D} 
%(Defined(e) $ $\cap \varphi(f_1)) \cup \bigcup_{e \in D} (Used(e) $ $
%\cap \varphi(f_2))$ 

%
By the above definition, we only represent the interaction between a 
pair of features because the interaction between more than two 
features is still represented by the interactions of pairs features. 
Indeed, assuming that there exists an interaction among $m > 2$ 
features. For simplicity, we consider the case of m = 3, $f_1$, 
$f_2$, and $f_3$, and $E_1$, $E_2$, and $E_3$ are the sets of share 
program entities of three pairs of features ($f_1$, $f_2$), ($f_2$, $f_3$), and ($f_3$, $f_1$).
%
If there exists a common entities shared between all these features, 
the interaction of them is still represented through the interactions 
of the pairs.
%
On the other case, there is no shared entity between all features, 
assuming that $E_1 \cap E_3 = \emptyset$. Since the functionality 
offered by $f_3$ is influenced by $f_1$\footnote{because the roles of 
$f_1$ and $f_3$ in this case are equal} through $f_2$, there exists 
an entity $e_1 \in def(f_1)$ whose value affects another entity $e_3 
\in use(f_3)$ by value propagation function, $p$, such that $e_3 = 
p(e_1)$. Hence, by identifying feature interactions between pairs, 
the interactions among more than two features are still captured. 
%

In highly configurable systems, most of reported bugs  are 
configuration-dependent faults that are only exposed under a set of 
certain configurations \cite{Abal:2018} \cite{Garvin:2011}. 
%Configuration-dependent Fault
\begin{definition}{({\bf Configuration-dependent Fault}).}
Given a configurable system, a fault of the system is considered as a 
configuration-dependent bug if only if there are two sets of
configurations $CP$ and $CF$, where $CP, CF \subsetneq \mathbb{C}$, such 
that all configurations in $CP$ execute as expected, while all 
configurations in $CF$ reveal the bug.
\end{definition}
%
For example, the bug in the Fig.~\ref{example_bug} is revealed only in
the configuration in which features \texttt{LOCKDEP}, \texttt{PPC\_256K
\_PAGES}, \texttt{\!SLOB}, and \texttt{SLAB} are all enabled and 
\texttt{PPC\_16K\_PAGES} is disabled. In 
practice, a configuration-dependent bug can be revealed during testing 
process, when there are configurations failing at least one test, 
while others pass all their test cases. Even after the system have been 
released, many configuration-dependent bugs are newly reported by the 
end-users when they execute the configurations in their own environments.
%

In fact, in a configurable code containing a configuration-dependent
bug, not all features are relevant to the visibility of the bug. Yet,
there are certain features that are enabled or disabled, in which the
bug is revealed during executing/testing every configuration
containing these feature selections. For example, in
Fig.~\ref{example_bug}, the bug is only triggered by the set of
enabled features including \texttt{LOCKDEP},
\texttt{PPC\_256K\_PAGES}, \texttt{\!SLOB}, and \texttt{SLAB}, along
with the disabling of \texttt{PPC\_16K\_PAGES}. The bug is invisible
if \texttt{PPC\_16K\_PAGES} is enabled.

%Suspicious PC
\begin{definition}{({\bf Fault-causing Partial Configuration}).}
Given a configurable system containing configuration-dependent bugs, the 
fault-causing partial configuration $PC$ of a particular configuration-
dependent bug is the non-empty smallest set of feature selections, such 
that $\forall c \in \mathbb{C}, c \supseteq PC \implies c \in CF$, where 
$CF$ is the set of configurations that reveal the bug.
\end{definition}

For example, the fault-causing partial configuration of the bug in shown in figure \ref{example_bug} is \{\texttt{SLAB=T}, \texttt{PPC\_16K\_PAGES=F}, \texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{\!SLOB=T}\}.
%

Assuming that in a buggy configurable code, $PC$ is the fault-causing partial configuration of exactly $N$ configuration-dependent bugs ($B$), and $FS$ is the set of features whose selection is in $PC$. We have the following theorem:

\begin{theorem}{({\bf Suspicious statements}).} The suspicious statements are the executed statements in the failed configurations that have dependency impact on the implementation of the interactions between the features $FS$.
\end{theorem}

\textbf{Proof}. First, the bug must be related to the statements that implement the interaction between features in $FS$ ($SS$). Indeed, if there exists a bug in $B$ that is caused by a statement $s$ in $FS$ but $s \not \in SS$, there exists a set.  In the running example, they are statements at lines 11, 12, 16, 22 (\texttt{i < PAGE\_SHIFT + MAX\_ORDER}) and 24.


==> implementation.tex <==
\section{Implementation}

==> interaction_algorithm.tex <==
\begin{algorithm}
\caption{{\tool}: Suspicious partial configuration detection}	
 \label{alg_1}
\begin{algorithmic}[1]
\Procedure {DetectSuspiciousPC}{$CP$, $CF$}
\State $partialConfig = EmptySet$
\State $consideredSels = commonSubSet(CF)$
%\State $unrelatedFeatures = FindUnrelatedFeatures(CF)$

%\ForAll {$f \in unrelatedFeatures$}
%	\State $enabledSel = enable(f)$
%	\State $disabledSel = disable(f)$
%	\State $remove(consideredSels, enabledSel)$
%	\State $remove(consideredSels, disabledSel)$
%\EndFor

\ForAll {$s \in consideredSels$}
	\State $subset = subtraction(consideredSels, s)$
	\ForAll {$passedConfig \in CP$}
		\If {$containAll(passedConfig, subset)$}
			\State $addToSet(selection, partialConfig)$
			\State $break$
		\EndIf
	\EndFor
\EndFor
\EndProcedure
\Statex

%\Procedure {FindUnrelatedFeatures}{$CF$}
%\State $unrelatedFeatures = EmptySet$
%
%\ForAll {$f \in AllFeatures$}
%	\State $enabledSel = enable(f)$
%	\State $disabledSel = disable(f)$
%	\State $config = findContainingConfig(enabledSel, CF)$
%	\State $other = findContainingConfig(disabledSel, CF)$
%	\If {$config \neq NULL \wedge other \neq NULL$ }
%		\State $addToSet(f, unrelatedFeatures)$
%	\EndIf
%\EndFor
%\EndProcedure
%\Statex
\end{algorithmic}
\end{algorithm}

==> interaction_detection.tex <==
\section{Suspicious feature interaction detection}
\label{interaction_detection_section}

For a suspicious partial configuration, $SPC$, {\tool} detects the interactions among the features whose selection in the $SPC$ that affect the visibility of the bugs in the configurations containing the $SPC$. 

In the configurable code, a feature is realized using the statements that operate (e.g., declare, define, refer, etc.) on the data structures and program entities (e.g., variables, functions). Thus, the interaction among features occurs when their statements operate on the program entities that are shared between those features. Let us provide our formulation on program entity, operation, and feature interaction.
%
\input{interaction_formulation}

\input{feature_interaction_algo}



==> interaction_dt.tex <==
\section{Suspicious feature interaction detection}
%Entity
In a program, we are interested in the program entities and the
operations that are performed on them.
\begin{definition}{({\bf Program Entity}).}
A program entity is a program element uniquely identified with
a \textit{name} and a \textit{scope}.
\end{definition}

In our formulation, we are interested in two types of program
entities: {\em variable} and {\em function}.
%
An entity is represented in the form of \texttt{[scope.ent\_name]},
where \texttt{scope} and \texttt{ent\_name} are the scope and the 
name of the program entity respectively. The \textit{scope} and the
\textit{name} of an entity are used together as the identity of the
entity. For example, the code in Fig.~\ref{example_bug} contains
variables \texttt{GLOBAL.kmalloc\_caches}, \texttt{init\_node
\_lock\_keys.i}, and function \texttt{GLOBAL.init\_lock\_keys}.
%

%Program Operation
In our work, there are two program operations on variables and
functions: \textit{define (def)} and \textit{use}. A \textit{def}
operation is used to \textit{assign} a value to a variable or
\textit{define} the body for a function. Meanwhile, a variable is
\textit{used} when it is \textit{used} or \textit{referred} to. A
function is \textit{used} if it is \textit{called}/\textit{invoked} or
used as a function pointer (C/C++). For example, the function
\texttt{GLOBAL.init\_node\_lock\_keys} is \textit{defined} as a set of
statements from lines 21--26 and \textit{called/used} in the statement
at line 33. For a variable \texttt{X}, it might be \textit{declared}
or \textit{destructed}. However, without loss of generality, when
\texttt{X} is declared or destructed, we consider that it is
\textit{defined} with \texttt{UNINIT} or \texttt{UNDEFINED} respectively. For instance, the value of
\texttt{init\_node\_lock\_keys.i} is \texttt{UNDEFINED} at line 21.
%

%Implementation Functions
Given a program, we define 2 \textit{implementation functions} as 
the functions from $E$ to $2^S$, where $E$ is the set of program 
entities, and $S$ is the set of statements of the program:
\begin{definition}{({\bf Implementation Functions}).}
\begin{itemize}[leftmargin=4mm]
  \item $Defined:E \to 2^S$, $Defined(e)$ is the set of statements that 
  implement the {\bf definitions} of $e$
  \item $Used:E \to 2^S$, $Used(e)$ is the set of statements that 
  implement the {\bf uses} of $e$
\end{itemize}
\end{definition}
In Fig.~\ref{example_bug},
$Defined($\texttt{GLOBAL.kmalloc\_caches}$)$ contains only statements
at line 16, while, the statement at line 24 is the only element of
$Used($\texttt{GLOBAL.kmalloc\_caches}$)$. For the compound
statements, we also consider the conditional expressions (\textit{if-statement}, \textit{for-loop}, \textit{while-loop} and \textit{do-loop}), the control expressions or the options (\textit{switch-statement}) and take them into account for localizing bugs.
%
% Break flow

%

%
%In practice, a feature (parent-feature) might contain several other features 
%(child-features). For example,...

%Feature
\begin{definition}{({\bf Feature-related Functions}).}
In a configurable system, which are implemented by a set of statements 
$S$ and consists of a set of features $F$ and a set of program 
entities $E$, we define two feature-related functions:
\begin{itemize}[leftmargin=4mm]
	\item $def:F \to 2^P$, $\forall e \in P, e \in def(f) 
	\Leftrightarrow 	Defined(e) $ $\cap \quad \varphi(f) \neq \emptyset$. 
	$def(f)$ is the set of program entities which are defined within 
	$f$, e.g., \texttt{cpuup\_prepare.node} $\in def($\texttt{NUMA}$)$; 
	%	
	or for functions, $f$ is used to realize their definition. For instance, since the statement at line 31 in \texttt{NUMA} is used to realize \texttt{GLOBAL.cpuup\_prepare}, this entity is also an element of $def($\texttt{NUMA}$)$.

	\item $use:F \to 2^E$, $\forall e \in P, e \in use(f)
	\Leftrightarrow Used(e) $ $\cap \quad \varphi(f) \neq \emptyset$. 
	$use(f)$ is the set of program entities that are used within $f$, 
	e.g., \texttt{GLOBAL.PAGE\_SHIFT}, \texttt{GLOBAL.kmalloc\_caches},~\texttt{GLOBAL.slab\_set\_lock\_classes} $\in use($\texttt{LOCKDEP}$)$.
	
%  \item $children: F \to 2^F$, $children(f)$ is the set of features that are 
%  child-features of $f$
%  \item $parent: F \to F$, $parent(f)$ the feature that $f$ is one of child-features of
\end{itemize}
\end{definition}
%
%
%\textit{The core feature}, $\Omega$, has no parent-feature, while every feature is
%contained by another one. If a (parent) feature is disabled, its child-features 
%are also disabled, and if one of child-features of a feature is enabled, the 
%feature is also enabled.

In a configurable system, two features can interfere each other 
through the program entities that are shared to implement these 
features. In the running example, \texttt{LOCKDEP} \textit{uses} 
\texttt{PAGE\_SHIFT} (line 22) and \texttt{kmalloc\_caches} (line 24) 
that are \textit{defined} by \texttt{SLAB} (line 11) and 
\texttt{!SLOB} (line 16) respectively to implement its functionality.
Hence, the optional functionality offered by \texttt{LOCKDEP} is
influenced when \texttt{SLAB} or \texttt{!SLOB} are enabled/disabled.
%
%
In this work, we focus on the feature interactions through shared 
program entities. The interactions associated with external data such 
as files or database are beyond the scope of this work. If both 
features \textit{use} a program entity, they will not change the 
program's state. By that our assumption, there is no interaction 
between two or more features if they only \textit{use} the same 
program entities. 
%The feature interaction between two features through 
%shared entities and $def$ and $use$ is described by the following 
%definition.

%
%Feature Interaction
\begin{definition}{({\bf Feature Interaction}).}
The interaction between two features $f_1$ and $f_2$ exists if only if 
$def(f_1) \cap def(f_2) \neq \emptyset$ (def-def) or $def(f_1) \cap use(f_2) \neq \emptyset$ (def-use). The statements that implement the definitions of the shared entities in $f_1$ and $f_2$ (def-def) and the uses of the share entities in $f_2$ (def-use) are the statements that implement the interactions.
\end{definition}
%

By the above definition, we only represent the interaction between a 
pair of features because the interaction between more than two 
features is still represented by the interactions of pairs features. 
Indeed, assuming that there exists an interaction among $m > 2$ 
features. For simplicity, we consider the case of m = 3, $f_1$, 
$f_2$, and $f_3$, and $E_1$, $E_2$, and $E_3$ are the sets of share 
program entities of three pairs of features ($f_1$, $f_2$), ($f_2$, $f_3$), and ($f_3$, $f_1$).
%
If there exists a common entities shared between all these features, 
the interaction of them is still represented through the interactions 
of the pairs.
%
On the other case, there is no shared entity between all features, 
assuming that $E_1 \cap E_3 = \emptyset$. Since the functionality 
offered by $f_3$ is influenced by $f_1$\footnote{because the roles of 
$f_1$ and $f_3$ in this case are equal} through $f_2$, there exists 
an entity $e_1 \in def(f_1)$ whose value affects another entity $e_3 
\in use(f_3)$ by value propagation function, $p$, such that $e_3 = 
p(e_1)$. Hence, by identifying feature interactions between pairs, 
the interactions among more than two features are still captured. 
%


Assuming that in a buggy configurable code, $PC$ is the fault-causing partial configuration of exactly $N$ configuration-dependent bugs ($B$), and $FS$ is the set of features whose selection is in $PC$. We have the following theorem:

\begin{theorem}{({\bf Suspicious statements}).} The suspicious statements are the executed statements in the failed configurations that have dependency impact on the implementation of the interactions between the features $FS$.
\end{theorem}

\textbf{Proof}. First, the bug must be related to the statements that implement the interaction between features in $FS$ ($SS$). Indeed, if there exists a bug in $B$ that is caused by a statement $s$ in $FS$ but $s \not \in SS$, there exists a set.  In the running example, they are statements at lines 11, 12, 16, 22 (\texttt{i < PAGE\_SHIFT + MAX\_ORDER}) and 24.




For each given the detected suspicious partial configuration 
$\mathbb{P}$, we statically analyze the features\footnote{DO WE 
NEED TO EXPLAIN WHY STATICALLY?} whose selection is an element of $
\mathbb{P}$ to detect the implementation of the interactions between those features in pairs, a set of statements $\mathbb{S}$. For a pair of features, we use algorithm \ref{alg_2} to detect the interaction between them. First, the algorithm identifies their shared program entities, which might (re-) defined by the two features or defined by a feature and used by other (lines 3, 4). After that, those shared entities are used to detect the set of statements ($interactionImpl$) that implement their definitions (lines 5 to 9) and those entities' definitions and uses (lines 10 to 14) in the two features.

\input{alg_2}

For example, by algorithm \ref{alg_2}, the set of statements that 
implement the interaction between \texttt{!SLOB} and 
\texttt{LOCKDEP} through \texttt{kmalloc\_caches} contains the 
statements at line 16 where \texttt{kmalloc\_caches} is defined and 
line 24 which uses the entity.

==> interaction_formulation.tex <==
\subsection{Formulation}
%Entity
\begin{definition}{({\bf Program Entity}).}
A program entity is a program element uniquely identified with
a \textit{name} and a \textit{scope}.
\end{definition}

In our formulation, we are interested in two types of program
entities: {\em variable} and {\em function}.
%
An entity is represented in the form of \texttt{[scope.ent\_name]},
where \texttt{scope} and \texttt{ent\_name} are the scope and the 
name of the program entity respectively. The \textit{scope} and the
\textit{name} of an entity are used together as the identity of the
entity. For example, the code in Fig.~\ref{example_bug} contains
variables \texttt{GLOBAL.kmalloc\_caches}, \texttt{init\_node
\_lock\_keys.i}, and function \texttt{GLOBAL.init\_lock\_keys}.
%

%Program Operation
In our work, there are two {\bf program operations} on variables and
functions: \textit{define (def)} and \textit{use}. A \textit{def}
operation is used to \textit{assign} a value to a variable or
\textit{define} the body for a function. Meanwhile, a variable is
\textit{used} when it is \textit{used} or \textit{referred} to. A
function is \textit{used} if it is \textit{called}/\textit{invoked} or
used as a function pointer (C/C++). For example, the function
\texttt{GLOBAL.init\_node\_lock\_keys} is \textit{defined} as a set of
statements from lines 21--26 and \textit{called/used} at line 33. For 
variable \texttt{X}, it might be \textit{declared}
or \textit{destructed}. However, without loss of generality, when
\texttt{X} is declared or destructed, we consider that it is
\textit{defined} with \texttt{UNINIT} or \texttt{UNDEFINED}
respectively. For instance, the value of
\texttt{init\_node\_lock\_keys.i} is \texttt{UNINIT} at line 21.
%
%Implementation Functions

Given a program, $\mathbb{E}$ is the set of program entities, 
and $\mathbb{S}$ is the set of statements of the program, we use 2
\textit{implementation functions} to map each entity in $\mathbb{E}$ 
to the sets of statements in $\mathbb{S}$ that implement its 
definitions and uses:
\begin{definition}{({\bf Implementation Functions}).}
\begin{itemize}
  \item $Define:\mathbb{E} \to 2^\mathbb{S}$, $Define(e)$ is the set of 
  statements that implement the {\bf definitions} of $e$
  \item $Use:\mathbb{E} \to 2^\mathbb{S}$, $Use(e)$ is the set of statements 
  that implement the {\bf uses} of $e$
\end{itemize}
\end{definition}
In Fig.~\ref{example_bug},
$Define($\texttt{GLOBAL.kmalloc\_caches}$)$ contains only statements
at line 16, while, the statement at line 24 is the only element of
$Use($\texttt{GLOBAL.kmalloc\_caches}$)$. For compound
statements, we also consider the conditional expressions
(\textit{if-statement}, \textit{for-loop}, \textit{while-loop} and
\textit{do-loop}), the control expressions or the options
(\textit{switch-statement}), and take them into account for localizing
bugs.

\begin{definition}{({\bf Propagation Function}).}
$\rho: \mathbb{E} \times \mathbb{C} \to 2^\mathbb{E}$, $\rho(e)$ 
is the set of program entities whose definition value/body is propagated to $e$, such that:
\begin{itemize}
	\item $\forall e_1 \in \mathbb{E}, use(e_1) \cap def(e) \cap \varphi(c) \neq \emptyset \implies e_1 \in \rho(e, c)$, or
	
	\item $\forall e_2 \in \mathbb{E}, \exists e_1 \in \rho(e, c), use(e_2) \cap def(e_1) \cap \varphi(c) \neq \emptyset \implies e_2 \in \rho(e, c)$
\end{itemize}
\end{definition}

where $\varphi(c) = \bigcup_{\substack{(f=T) \in c}} \varphi(f)$. For the 
running example, $\rho($\texttt{init\_}-\texttt{node\_lock\_keys.lock}$, c_2)=\{$\texttt{init\_node\_lock\_keys.node}, \texttt{GLO}-\texttt{BAL.slab\_set\_lock\_classes}$\}$, 
or another example is that $\rho($\texttt{GLO}-\texttt{BAL.cpuup\_prepare}$, c_3)$ 
contains functions \texttt{init\_node\_lock\_keys} and \texttt{slab\_set\_lock\_classes}.

%Feature
\begin{definition}{({\bf Feature-related Functions}).}
In a configurable system, which is implemented by a set of statements 
$S$ and consists of a set of features $F$ and a set of program 
entities $E$, we define two feature-related functions:
\begin{itemize}
	\item $def:\mathbb{F} \to 2^\mathbb{E}$, $\forall e \in \mathbb{E}, e \in def(f) 
	  \Leftrightarrow Define(e) $ $\cap \quad \varphi(f) \neq \emptyset$. 
	  That is, if the set of statements implementing the definitions of $e$ 
	  overlaps with the set of statements realizing the feature $f$, then $e$ 
	  belongs to $def(f)$. For variable, $def(f)$ is the set of variables 
	  which are defined within $f$, e.g., \texttt{cpuup\_prep}-\texttt{are.node} 
	  $\in def($\texttt{NUMA}$)$.
	%	
	For function, $f$ is used to realize their definition. For instance, since 
	the statement at line 31 in \texttt{NUMA} is used to define the body of 
	\texttt{GLOBAL.cpuup\_prepare}, this entity is also an element of $def($\texttt{NUMA}$)$.

	\item $use:\mathbb{F} \to 2^\mathbb{E}$, $\forall e \in \mathbb{E}, e \in use(f)
          \Leftrightarrow Use(e) $ $\cap \quad \varphi(f) \neq
          \emptyset$.  That is, if the set of statements~implementing
          the uses of $e$ overlaps with the set of statements realizing the 
          feature $f$, then $e$ belongs to $use(f)$.
          %
	Specifically, $use(f)$ is the set of program entities~that are used within $f$, 
	e.g., \texttt{GLOBAL.PAGE\_SHIFT}, \texttt{GLOBAL.kmalloc\_cach\-es},
	~\texttt{GLOBAL.slab\_set\_lock\_classes} $\in use($\texttt{LOCKDEP}$)$.
	
\end{itemize}
\end{definition}

In a configurable system, two features can interfere or influence each other 
through the program entities that are related to these 
features. In the running example, \texttt{LOCKDEP} \textit{uses} 
\texttt{PAGE\_SHIFT} (line 22) and \texttt{kmalloc\_caches} (line 24) 
that are \textit{defined} by \texttt{SLAB} (line 11) and 
\texttt{!SLOB} (line 16) respectively to implement its functionality.
Hence, the optional functionality offered by \texttt{LOCKDEP} is
influenced when \texttt{SLAB} or \texttt{!SLOB} are enabled/disabled.
%
%
In this work, we focus on the feature interactions through program entities. The interactions associated with external data such as files or database are beyond the scope of this work. By that our assumption, if both features \textit{use} program entities, they will not change the program's state. Therefore, there is no feature interaction related to program entities that are only \textit{used} by features. 

%
%Feature Interaction
\begin{definition}{({\bf Feature Interaction}).}
The interaction between two features $f_1$ and $f_2$ exists if:
\begin{enumerate}
	\item $\exists e \in \mathbb{E}$, such that $ e \in def(f_1) \cap def(f_2)$, or
	\item $\exists e_1 \in def(f_1), e_2 \in use(f_2)$ such that $e_1 \in \rho(e_2, c)$, or
	\item $\exists e_1 \in use(f_1), e_2 \in def(f_2)$ such that $e_2 \in \rho(e_1, c)$
\end{enumerate}
\end{definition}
%
where $c$ contains both $(f_1=T)$ and $(f_2=T)$. For (1), the intuition is that if a program entity is defined by a feature, this entity then is re-defined by another feature, then there exists an interaction among those features. For (2) and (3), if there is an entity defined by feature $f$, its value is propagate to another entities that are used by feature $f'$. This means $f'$ is influenced by $f$, and they interact. In this definition, $e$, $e_1$, and $e_2$ are related to the feature interaction among $f_1$ and $f_2$
%

By the above definition, we only represent the interaction between a pair of features because the interaction between more than two features is still represented by the interactions of pairs features. Indeed, assuming that there exists an interaction among $m > 2$ features. For simplicity, we consider the case of $m = 3$ features, $f_1$, $f_2$, and $f_3$, the interactions between pairs of features include ($f_1$, $f_2$), ($f_2$, $f_3$), and ($f_3$, $f_1$). Since the functionality offered by $f_3$ is influenced by $f_1$\footnote{because the roles of $f_1$ and $f_3$ in this case are equal} through $f_2$, there exists a program entity $e_1 \in def(f_1)$ whose value/body is propagated to another program entity $e_3 \in use(f_3)$, $e_1 = \rho(e_3)$. Hence, by identifying interactions between pairs of features, the interactions among more than two features are still captured. 
%
%
\begin{definition}{({\bf Feature Interaction Implementation}).} 
The implementation of the interaction between features $f_1$ and $f_2$ are the statements that implement the definitions of the shared entities in $f_1$ and $f_2$ (for def-def interactions) and the uses of the shared entities in $f_1$ and $f_2$ (for def-use interactions).
\end{definition}



==> intro.tex <==
\section{Introduction}
\label{sec:intro}
\textit{Highly-configurable system} supports the diversification of
software products by providing a large number of \textit{configuration
  options} that are used to control different \textit{features}. The
features are implemented as optional blocks of code and can be
configured to meet the requirements of a wide range of
customers. However, this also induces challenges in program analyses
and quality assurance~\cite{productlinesbook1, productlinesbook2,
  productline_survey}.

%
In configurable systems, most faults are \textit{configuration-dependent 
faults}~\cite{Garvin:2011, plugin_testing, Kuhn:2004, Yin:2011, 
medeiros2015love}, which cause the failures in only certain configurations 
because of \textit{feature interactions} \cite{plugin_testing, 
Abal:2018, Garvin:2011}. Manually localizing configuration-dependent 
fault in buggy configurable systems could be extremely time-consuming 
due to their complexity~\cite{Meinicke:2016, productline_survey}.
%
Meanwhile, exiting automated fault localization techniques 
\cite{wong2009survey} focus on localizing bugs in particular buggy 
configurations. Specifically, they do not consider the configurability 
dimension of configuration-dependent fault: A statement that is run in 
faulty configurations may be also executed as expected. As results, they 
might not provide a thorough evaluation for statements in a buggy 
configurable system.
%
%Even after the system have been released, many configuration-dependent
%bugs are newly reported by the end-users when they execute the
%configurations in their own environments.
%
%* Localizing normal bug is time-consuming, for configuration-dependent fault, 
%it is much more expensive because of the complexity 
%
Though spectrum-based techniques such as Tarantula~\cite{tarantula} 
can be used on configurable code by considering options 
as conditions, these approaches access statements based on their 
execution information and lack the consideration of the meaning of 
statements in configurable code. Consequently, they provide the same 
suspiciousness assessment to every statement that have similar 
execution patterns~\cite{Pearson:2017}. For example, since options are 
considered as program conditions, they might assign the same 
suspiciousness level to all statements in the whole feature. That makes 
configuration-dependent fault localizing becomes extremely inefficient~
\cite{Pearson:2017, exam, wong2009survey}. This inefficiency will be
illustrated in the next section.
%
%

In this work, to address this problem of configuration-dependent fault
localization, we propose {\tool}, a novel approach to localize
configuration-dependent bugs in configurable systems. The inputs of
our algorithm include a buggy configurable system, the set of its
tested configurations including passed configurations and the
configurations that are failed at least one test, and the execution
information collected during the testing phase. {\tool} analyzes
the test results, the code, and the execution information to isolate
the statements that are most likely to be buggy and provide a
suspiciousness assessment for each of them.
%
For a buggy configurable system, localizing the bug in the system
should be started from the set of features (called \textit{suspicious 
features}) whose combination reveals the failure in all failed 
configurations. For example, all configurations which enable two 
suspicious features \texttt{A} and \texttt{B} are failed at
least one test, while every configuration where each of them is
switched to be disabled behaves as expected. In fact, the unexpected
behaviors of the failed configurations are caused by the interaction of
those suspicious features (called \textit{suspicious feature
  interaction}) that perform \textit{program operations} (e.g.,
declarations, references, assignments, etc) on the shared \textit{data
  structures/program entities} (e.g., variables, functions,
etc.). Hence, every executed statement that has certain impact on the
suspicious interaction should be considered as a \textit{suspicious
  statement}.
%

Specifically, in {\tool}, with the test results of all configurations,
we analyze to detect the set of suspicious features which are
enabled/disabled in all failed configurations, and their switching
makes the resulting configuration pass all the tests. Then, those
suspicious features are statically analyzed to detect the suspicious
interactions between them through program operations on the shared
data structures/program entities. These suspicious interactions are
used to identify the suspicious statements that are the executed
statements having dependency impact on the interactions. Finally, the
suspicious statements are ranked according to suspiciousness assessed
using a spectrum-based method \cite{wong2009survey} based on their
execution information collected in the testing phase.


We evaluated the effectiveness of {\tool} in fault localizing artificial 
seeded configuration-dependent faults in a highly-configurable system. We 
evaluated the improvement when we run {\tool} with the state-of-the-art 
spectrum-based fault localization approach, Tarantula \cite{tarantula}, 
and Tarantula alone on the same set of artificial configuration-dependent 
bugs. We found that {\tool} significantly improves the baseline 
spectrum-based approach. By {\tool}, on average, the correctness in 
ranking the buggy statements increases more than \textbf{9} times, and 
the search space is significantly narrowed down, up to about \textbf{15} 
times. Additionally, we performed several experiments to evaluate the 
scalability of {\tool} in bug localization in the large-scale configurable 
systems.

In summary, in this paper, our main contributions are:
\begin{itemize}
\item A novel efficient configuration-dependent fault localization 
technique for configurable systems;
\item An empirical study showing the effectiveness and scalability 
of {\tool} in configuration-dependent fault localizing for large-scale 
configurable systems.
\end{itemize}


==> limitations.tex <==
\subsection{Limitations}

For the cases that {\tool} did not rank well the buggy configurations,
we found that the majority of them are not in the kinds of
interaction-related defects listed in Section~\ref{sec:formulation}.
%
As an example, a variable \texttt{x} is assigned
a value \texttt{v} if option \texttt{A} is enabled, otherwise
\texttt{x=v'}. Then, \texttt{x} is referred to in a feature controlled
by option \texttt{B}. In this case, {\tool} detects the
interactions between those features. However, as a static technique,
{\tool} could not conclude which option selections are more suspicious. That can be done by the dynamic approaches~\cite{icse14-varex}.

%
Figure~\ref{apache1} shows an example that {\tool} did not rank well the buggy configurations. In this example, a \textit{use 
without assignment} is exposed when \texttt{APU\_HAS\_LDAP} and 
\texttt{APU\_HAS\_SHARED\_MEMORY} are enabled. {\tool} did not work well in this 
example because there is no feature where \texttt{rmm\_lock} is assigned, 
consequently, no \textit{assign-use} interaction exists. 
However, {\tool} ranked the configuration that reveals the flaw 
\textit{unused variable} (\texttt{rmm\_lock}) when \texttt{APU\_HAS\_LDAP=T} and \texttt{APU\_HAS\_SHARED\_MEMORY=T}. {\bf What is conclusion?}
%

In X cases, the interactions that cause the interaction bugs are really 
detected, but the configurations that reveal the bugs are still ranked 
lower than others. The reason for these cases is that other 
configurations containing more suspicious selections that actually do not 
cause other bugs.


%linux_21
\begin{figure}[t]
\lstinputlisting[label=example_bad,captionpos=b]{example_bad.c}
\caption{An example that {\tool} did not rank well the buggy configurations}
\label{apache1}
\end{figure}


==> overview.tex <==
%\textbf{Overview.} Base on these observations, we propose an
%configuration-dependent fault localization approach that first analyze
%the test results of the given configurable code containing
%configuration-dependent bugs to identify a smallest set of features
%whose enabling/disabling make the bugs visible (\textbf{O1}). That helps us narrow
%down the search space for the buggy statements. Then,
%those features are statically analyzed to detect the statements that
%implement the interactions between them, and these statements are
%considered to be suspicious (\textbf{O2} and \textbf{O3}). Finally, the executed statements are
%analyzed to detect the statements that have impact on the suspicious
%statements, these s tatements are also suspicious (\textbf{O4}).

%\textbf{Overview}.

\subsection{Approach Overview}

Based on these observations, we propose, {\tool}, a novel approach for
configuration-dependent fault localization.  The input for {\tool}
includes the buggy configurable code, the~test result of each
configuration, and the trace of the executed~statements that are
recorded for each test in each configuration, e.g., the trace of the
executed statements in $c_7$ is shown in Fig.~\ref{execution_trace}.

\begin{figure}[h]
\centering
\includegraphics[width=0.47\textwidth]{flowchart}
\label{workflow}
\caption{{\tool}'s approach overview}
\end{figure}
%
In general, to localize a configuration-dependent bug, our algorithm
works in three steps as shown in Fig.~\ref{workflow}.

1) First, {\tool} aims to detect the set of features that have
potential interactions that could cause the configuration-dependent
faults and make the tests failed. Using all features in the feature
space would be inefficient. Thus, we aim to determine an optimal set of
such feature candidates whose enabling/disabling make the bug visible
(based on \textbf{O1}). The optimal set with the selections of
enabling/disabling of each feature must satisfy both necessity and
sufficiency conditions. The set is said to be {\em necessary} if and
only if for any strict subset of the set,
%
there exists a configuration that contains it and does not fail any
test. It is said to be {\em sufficient} if and only if~the selections
of other features outside of the set do not have any impact on the
test results (e.g., \texttt{NUMA}).
%
Let us call such a set the \textit{suspicious partial
  configuration (SPC)} (Section~\ref{SPC_detection_section}). For the
example, \{\texttt{SLAB=T}, \texttt{PPC\_16K\_PAGES=F},
\texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{!SLOB=T}\}
is considered as the SPC of the bug. $c_4$ has no failed tests because
\texttt{SLAB} is disabled (\texttt{SLAB=F}). the selections of
\texttt{NUMA} does not belong to the SPC of the bug because they do not 
have any impact on the visibility of the bug.


%To narrow down the search space, it first identifies a smallest set of
%feature candidates whose enabling/disabling (selections) make the bug
%visible (based on \textbf{O1}). The resulting set of feature
%selections is called the \textit{suspicious partial configuration
%(SPC)} that potentially causes the bug. Any configuration that
%contains a strict subset of SPC will be passed.
%
%For the running
%example, \{\texttt{SLAB=T}, \texttt{PPC\_16K\_PAGES=F}, \texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{\!SLOB=T}\}
%should be considered as the SPC of the bug. $c_4$ is passed because \texttt%{SLAB} is disabled (\texttt{SLAB=F}). The selections of other
%features do not have any impact on the visibility of the bug
%(e.g., \texttt{NUMA}).

\begin{figure}[h]
\begin{center}
\lstinputlisting[captionpos=b]{executed_stms.c}
\caption{The Trace of the Executed Statements in $c_7$}
\label{execution_trace}
\end{center}
\end{figure}

2) Next, {\tool} aims to detect the suspicious statements that are
responsible for feature interactions and potentially cause the
fault. To do that, it analyzes the features in SPC to detect the
interactions between them that are mostly likely to cause/disguise the
configuration-dependent bug. {\tool} then detects the statements that
realize those interactions (based on \textbf{O2} and \textbf{O3}). The
interactions are detected via the shared program entities controlled by
different features and the operations performed on them
(Section~\ref{interaction_detection_section}). Those statements in the
example are at lines 4, 11, 12, 16, 22, and~24.

%the features enabled/disabled in the SPC, whose interactions between
%them are most likely to cause/disguise the configuration-dependent
%bug, are analyzed to detect the statements that implement those
%interactions (based on \textbf{O2} and \textbf{O3}). Those statements
%in the example are the statements at lines 4, 11, 12, 16, 22, and 24.

3) Finally, these suspicious statements are used to
detect other suspicious statements that are executed and 
have dependency impact \cite{cia, pdg} on them in the failed 
configurations (based on \textbf{O3} and \textbf{O4}). The output for the 
running example is the set of statements at lines 11, 12,  22, 1, and 4.
%
%


==> partial_config_dt.tex <==
\section{Suspicious partial configuration detection}

In highly configurable systems, most of reported bugs  are 
configuration-dependent faults that are only exposed under a set of 
certain configurations \cite{Abal:2018} \cite{Garvin:2011}. 
%Configuration-dependent Fault
\begin{definition}{({\bf Configuration-dependent Fault}).}
Given a configurable system, a fault of the system is considered as a 
configuration-dependent bug if only if there are two sets of
configurations $CP$ and $CF$, where $CP, CF \subsetneq \mathbb{C}$, such 
that all configurations in $CP$ execute as expected, while all 
configurations in $CF$ reveal the bug.
\end{definition}
%
For example, the bug in the Fig.~\ref{example_bug} is revealed only in
the configuration in which features \texttt{LOCKDEP}, \texttt{PPC\_256K
\_PAGES}, \texttt{\!SLOB}, and \texttt{SLAB} are all enabled and 
\texttt{PPC\_16K\_PAGES} is disabled. In 
practice, a configuration-dependent bug can be revealed during testing 
process, when there are configurations failing at least one test, 
while others pass all their test cases. Even after the system have been 
released, many configuration-dependent bugs are newly reported by the 
end-users when they execute the configurations in their own environments.
%

In fact, in a configurable code containing a configuration-dependent
bug, not all features are relevant to the visibility of the bug. Yet,
there are certain features that are enabled or disabled, in which the
bug is revealed during executing/testing every configuration
containing these feature selections. For example, in
Fig.~\ref{example_bug}, the bug is only triggered by the set of
enabled features including \texttt{LOCKDEP},
\texttt{PPC\_256K\_PAGES}, \texttt{\!SLOB}, and \texttt{SLAB}, along
with the disabling of \texttt{PPC\_16K\_PAGES}. The bug is invisible
if \texttt{PPC\_16K\_PAGES} is enabled.

%Suspicious PC
\begin{definition}{({\bf Fault-causing Partial Configuration}).}
Given a configurable system containing configuration-dependent bugs, the 
fault-causing partial configuration $PC$ of a particular configuration-
dependent bug is the non-empty smallest set of feature selections, such 
that $\forall c \in \mathbb{C}, c \supseteq PC \implies c \in CF$, where 
$CF$ is the set of configurations that reveal the bug.
\end{definition}

For example, the fault-causing partial configuration of the bug in shown in figure \ref{example_bug} is \{\texttt{SLAB=T}, \texttt{PPC\_16K\_PAGES=F}, \texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{\!SLOB=T}\}.



The bugs in the failed configurations might be caused by different 
fault-causing partial configurations. Hence, in this phase, we use 
test results to identify the suspicious partial configuration that 
causes the bugs in each failed configuration. 
%
\textit{For simplicity, we assume that all configuration-dependent
  bugs in the system are independent.} This implies that there is no
configuration that contains multiple bugs and passes all tests.
%

Given $CP$ and $CF$ that are sets of passed configurations and failed
configurations respectively, each failed configuration in $CF$ reveals
certain $k$ bugs, and each bug $i^{th}$ has its own fault-causing
partial configuration, $PC_i$. Hence, if every configuration
$c$, such that $c \supset \bigcup {PC_i} = P$, then $c \in CF$.  We
have the following properties about $P$:
%
%\begin{property}
%\label{proper_1}
%For a particular failed configuration $c \in CF$, $\forall s_1, s_2 
%\neq \emptyset$, $s_1 = c \backslash s_2$, if $\exists c' \in CP$, 
%such that $s_1 \subset c'$, then $s_1 \cap P \neq \emptyset \wedge 
%s_2 \cap P \neq \emptyset$.
%\end{property}

\begin{property}
\label{proper_1}
For a set of feature selections $S$, $S\supseteq P$, $\forall s_1, s_2 
\neq \emptyset$, $s_1 = S \backslash s_2$, if $\exists c' \in CP$, 
such that $s_1 \subset c'$, then $s_2 \cap P \neq \emptyset$.
\end{property}

%
In other words, for a set of feature selections $S$ containing $P$, if 
a subset of $c$, $s_1$, is a part of a passed configuration $c'$, 
which means $s_1$ does not contain any full fault-causing partial 
configuration, then $s_2$ contains a subset of $P$.
%

The following property is a special case of property \ref{proper_1} 
when $s_2$ contains only one selection.

\begin{property}
\label{proper_2}
For a set of feature selections $S$, $S\supseteq P$, if $\forall s \in 
S$, $\exists c' \in CP$, such that $S \backslash s \subset c'$, then $s \in P$.
\end{property}

In the running example, by property \ref{proper_2}, for the bug revealed in $c_2$ containing a fault-causing partial configuration, selection $s=$\texttt{(SLAB=T)} is an element of the fault-causing partial configuration because $c_2 \backslash s \subset c_4$ and $c_4$ is a passed configuration.
%

\input{single_bug}


==> pc_detection.tex <==
\section{Suspicious partial configuration detection}
\label{SPC_detection_section}

For a buggy system, whose sets of passing and failing configurations
are $CP$ and $CF$ respectively, our first step is to detect the {\em
  optimal set of feature selections} that makes any configuration
containing it fail at least a test. We called this set the {\em
  suspicious partial configuration} ($SPC$) of the faults whose
visibility is affected by the interactions among the features selected
in $SPC$. That is, interactions among the features selected in 
$SPC$ cause the faults that we are detecting.

%
In fact, the unexpected interaction among features selected in a single
$SPC$ might cause more than one bugs. Meanwhile, a single 
configuration-dependent fault can be revealed by multiple $SPC$s.

\subsection{Suspicious Partial Configuration (SPC)}
 
A set of feature selections, $S$, is considered as a $SPC$ if and only 
if $S$ satisfies both the following necessity and sufficiency conditions.

\begin{definition}{({\bf Necessity}).}
$\forall c \in \mathbb{C}$, $c \supseteq S \implies c \in CF$, where 
$\mathbb{C}$ is the set of available configurations.
\end{definition}

That is, {\bf any configuration that contains $S$ would behave
unexpectedly, i.e. fail at least one test}.  In
Table~\ref{test_results}, $S_1=$\{\texttt{PPC\_16K\_\-PAGES=F},
\texttt{SLAB=T}, \texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T},
\texttt{!SLOB=T}\} satisfies the necessity condition, while
$S_2=$\{\texttt{SLAB=T}, \texttt{LOCKDEP=T}\} does not satisfy the
condition since $S_2$ is contained by $c_5$ and $c_3$ that pass all
tests.
% Tien
If the necessity condition were not satisfied, i.e., if there existed a
configuration containing $S$ and passing all the tests, the
interactions among the features selected in $S$ would have been
insufficiently to reveal any bug.
%
For example, for $S_2$, the interaction between \texttt{SLAB} and
\texttt{LOCKDEP}, which are the features in $S_2$, is not
sufficient to reveal any bug. Thus, we need the necessity~condition.
%
%Tien
%From the necessity condition, we can state that {\em if there exists a
%  configuration that contains $S$ and passes all the tests, the
%  interactions among the features selected in the set $S$ do not
%  affect the visibility of any bug, i.e., do not reveal any bug}.

%


\begin{definition}{({\bf Sufficiency}).}
$\forall c' \in \mathbb{C}$, $c' \in CP \implies c' \not \supset S$, 
where $\mathbb{C}$ is the set of all tested configurations.
\end{definition}

In other words, {\bf $S$ is not contained by any configuration that passes
  all the tests}.
%
In Figure~\ref{test_results}, $S_1$, $c_2$ and $c_7$ satisfy the
sufficiency condition.
%Tien
If the sufficency condition were not satisfied, i.e., there existed a
configuration containing $S$ and passing all the tests, the
interactions among the features selected in $S$ would have been
already validated, i.e., would not cause any bug. Thus, we need the
sufficency condition.
%
%From the definition, {\em if there is a passing
%  configuration that contains $S$, the interactions among the features
%  whose selections in $S$ is already validated and does not cause any
%  fault}. 

In general, the goal of Fault Localization is to help developers find
a good starting point to initiate the bug-fixing process rather than
provide a complete set of code that must be
fixed~\cite{wong2009survey}. With this goal, we want to have a set of
selections that satisfies both necessity and sufficency conditions and
is mimimal.
%
%if a set of selections and its subset that both satisfy the necessity
%and sufficiency conditions, the smaller set should be
%investigated.
For instance, although $S_1$, $c_2$ and $c_7$ satisfy
the sufficiency condition, since $c_2, c_7 \supset S_1$, $S_1$ is
considered as the only $SPC$ of the system in the running
example. Thus, $S$ is considered as a $SPC$ if it satisfies the
minimal condition:
\begin{definition}{({\bf Minimality}).}
$\not \exists S', S' \subset S$, and $S'$ satisfies both the necessity 
and sufficiency conditions.
\end{definition}



\input{properties}



\input{alg_1.5}

\subsection{$SPC$ Detection Algorithm}

Listing~\ref{alg_1_5} describes our algorithm to detect suspicious
partial configurations in buggy configurable code given $CP$ and $CF$,
which are sets of available passing and failing configurations
respectively.

In Algorithm~\ref{alg_1_5}, for each configuration $c$ that fails at
least one test, we aim to compute the list of $SPC$ sets. According to
Property 1, to do that, we compute $\wp$ that contains the sets of
feature selections such that for each set of selections, when all
selections in that set are reversed, the resulting configuration
passes all the tests (Property \ref{proper_2}). For efficiency, 
we consider each of the passing configurations $c'$ in $CP$ (line 5). 
We then compute the set $S$ of feature selections that were switched 
(line 6) to make $c$ become $c'$ (passing all the tests). If $S$ is 
non-empty, i.e., it is feasible to make such a switch, we will collect 
$S$ into the set $\wp$ (lines 7--8).
%
%
In $\wp$, for a set of selections, $S$, there could exist another set
of selection $S'$, where $S' \subset S$. This could lead to that $S$
might contain selections that do not reveal the bugs. Therefore, to
achieve minimality, we keep in $\wp$ the minimal set of feature
selections that have no subset in $\wp$ (line 9).
%
%According to Property 1, each of the sets $S$ in $\wp$ overlaps with
%every $SPC$ set, we compute the union set of feature selections
%$\partial$ as $\partial = \bigcup_{\substack{S \in \wp}} S$.
%
Then, $\wp$ is used to compute the union set of feature selections
$\partial$ as $\partial = \bigcup_{\substack{S \in \wp}} S$.
%
From lines 11--13, we identified the list of $SPC$ set by considering
all subsets of $\partial$ and collecting the ones satisfying both
necessity and sufficiency conditions and Property \ref{proper_2}.
%
%the $SPC$s in $c$ are identified by detecting all subsets of
%$\partial$ that satisfy the necessity and sufficiency conditions and
%Property \ref{proper_2} (line 11--13).
%
Finally, all the non-minimal sets are eliminated from the list of
$SPC$s according to the minimality condition (line 14).
%
%\input{alg_1}
%In the case of single $SPC$, instead of computing $S$ for every single the configuration $c$ at line 6, we examine the intersection of all configurations in $CF$ (Property \ref{proper_5}).
%
In Table~\ref{test_results}, the detected single suspicious partial
configuration by Algorithm~\ref{alg_1_5} is
\{\texttt{PPC\_16K\_PAGES=F}, \texttt{SLAB=T},
\texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{!SLOB=T}\}.


==> properties.tex <==
\subsection{Important Property to Detect $SPC$s}

%Before presenting how we construct $SPC$s, let us explain the following 
%important properties of $SPC$ that is useful in such construction. 

For a given configuration $c$ that fails at least a test, we aim to
identify one or more $SPC$ sets ($SPC \subset c$), i.e., one or more
sets of feature selections whose interactions are responsible for the
bugs causing the failure.
%Tien
%
In this section, we will show that to derive $SPC$s, we need to derive
the subsets $S$ of $c$ such that each of them satisfies the following
property:

%To detect the $SPC$s in a failing configuration, $c$, we aim to
%identify the sets of feature selections $S$ that are subsets of $c$,
%and each those sets of selections satisfies the following property:

\begin{property}
\label{proper_2}
For a failing configuration $c$, when all feature selections in $S$
are reversed/switched to the different values, the resulting
configuration $c'$ passes all the tests.
\end{property}

%Tien: don't know where to put this sentence
%The reason is that if $S$ has the Property \ref{proper_2}, then $S$
%must contain at least one feature selection in every $SPC$ of $c$.

Specifically, we will show the following theorem:

\begin{theorem}
\label{theorem_1}
%
The set $S$ of feature selections that satisfies
Property~\ref{proper_2} must contain at least one feature selection in
each $SPC$ for the failing configuration $c$.
\end{theorem}

\noindent {\bf Proof.}  Let us prove by contradiction. Assume that
$S$ has the property \ref{proper_2} and there exists a $SPC$ in $c$,
such that there is no feature selection in $SPC$ contained by $S$,
i.e., $S \cap SPC = \emptyset$.
%
%Tien
%
Since $SPC$ does not overlap with $S$, $SPC \supseteq T$ where $T = c
\backslash S$. In fact, $T$ is the set of feature selections in $c$
that are not switched and remained in $c'$, and $T \subset c'$.
%Thus, $SPC \supseteq T$, where $T = c \backslash S$ which is the set
%of feature selections in $c$ that are not switched and remained in
%$c'$, $T \subset c'$.
%
That leads to $c' \supset SPC$. According to necessity condition, we
have $c' \in CF$. This contradicts with the assumption. Therefore, $S$
must contain at least one feature selection in every $SPC$ of $c$.

As a result, if $S$ contains only one selection
$s$, then $s$ must be in $SPC$. The intuition is that if 
the selection of a feature affects the visibility of the bugs, 
this selection must be in the $SPC$.
%
For the failing configuration $c_2$, since selection 
$s=$\texttt{(SLAB=T)}, $c_2 \backslash \{s\} \subset c_4$, 
and $c_4$ passes all the test cases, \texttt{(SLAB=T)} is 
an element of the $SPC$. 

\noindent {\bf Implication.} By using Property \ref{proper_2}, for a
particular failing configuration $c$, we can identify $\wp$ which
contains all sets of feature selections having Property
\ref{proper_2}. Since every $S$ in $\wp$ contains at least one feature
selection in all $SPC$s of $c$, $SPC \subseteq \bigcup_{\substack{S
    \in \wp}} = \partial$ for every $SPC$ of $c$. This means that
$SPC$s need to be detected are subsets of $\partial$ that satisfy the
necessity, sufficiency and minimality conditions.

%In general, the principle of the 
%examining if a selection is an element of $SPC$ in Property 
%\ref{proper_2} can be applied for any set of selections 
%that contains $SPC$, not only failing configurations.
%

%In the case that the buggy system has a single $SPC$, the 
%unexpected behaviors in all failing configurations are 
%revealed by a single $SPC$, and $SPC$ is contained by all 
%failing configurations (the necessity). Therefore, we have 
%the following special property:
%
%\begin{property}
%\label{proper_5}
%In a buggy system has a single $SPC$, $SPC \subseteq \bigcap_{\substack{c \in CF}} c$.
%\end{property}


==> related.tex <==
\section{Related Work}
\label{related}
%Configuration-dependent bug: \cite{Garvin:2011}, \cite{Abal:2018}, \cite{plugin_testing}
%
%Failure-inducing Combination: \cite{failure_inducing_com}, \cite{buggy_interaction}
%
%Distinguish test failures caused by problems in test/code from those caused by illegal configurations \cite{Souto:2015}
%
%Traditional fault localization methods: \cite{tarantula}, \cite{ochiai} (survey: \cite{wong2009survey})
%
%Configuration Sampling: \cite{sampling}

%


Garvin and Cohen~\cite{Garvin:2011} have conducted an extensive
experiment to study configuration-dependent bugs. They reported that
that varying the system configuration amplifies the fault-finding
power of a test suite, making these faults easier to expose.  To help
in revealing those bugs, testing methods for configurable systems have
been proposed. In ~\cite{plugin_testing}, the authors revealed that in
testing plug-in-based systems, unit testing plays a key role, whereas
plug-in specific integration problems are identified and resolved by
the community.
%
%Based on that findings, Michaela Greiler \textit{et al.} proposed a
%series of recommendations and areas for future research.
In their recent study, Iago Abal \textit{et al.}~\cite{Abal:2018}
concluded that variability bugs are not confined to any particular
type of bugs, error-prone features, or specific locations.

Combinatorial testing has been shown to be a very effective testing
strategy. Based on a notion called failure-inducing combinations, the
result of combinatorial testing is improved
significantly~\cite{failure_inducing_com}. Zhang and
Zhang~\cite{buggy_interaction} proposed a new fault characterization
method called faulty interaction characterization (FIC) and its binary
search alternative (FIC\_BS) to locate one failure-causing interaction
in a single failing test case.

A software product line (SPL) is a family of programs that are
differentiated by features — increments in
functionality. SPLif~\cite{Souto:2015}, the first approach for testing
SPLs, uses a profile of passing and failing test runs to quickly
identify failures that are indicative of real problems in test or code
rather than specious failures due to illegal feature combinations.

The traditional fault localization method Tarantula \cite{tarantula}
uses color to visually map the participation of each program statement
in the outcome of the execution of the program with a test suite,
consisting of both passed and failed test cases to inspect and
identify statements involved in failures. Besides, using the type of
program spectra the Ochiai coefficient \cite{ochiai} consistently
outperforms those used in Pinpoint (Jaccard), Tarantula, and AMPLE in
software fault localization. 

An empirical investigation of the relationship between spectra
differences and regression faults revealed that certain types of
spectra differences correlate with high frequency—at least in one
direction—with the exposure of regression faults. That is, when
regression faults are revealed by particular inputs, spectra
differences are likely also to be revealed by those inputs, though the
reverse is not true \cite{sampling}.

There are several classes of fault localization methods for
traditional code. First, a class of spectrum-based, statistical
techniques~\cite{tarantula05,liblit-pldi05,santelices09}
%zhang-fse09}
applies statistical metrics on program entities based on their
coverage in passing and failing tests. Others analyze statistical
correlations between failure and CFG's
predicates~\cite{liblit-pldi05,sober05}, paths~\cite{holmes-icse09},
time spectra~\cite{timespectra08}, etc.
%code changes~\cite{stoerzer-fse06}. 
The second class relies on program~slicing~\cite{dor-issta08},
%such as static slicing~\cite{dor-issta08}, 
field-sensitive program
dependence~\cite{litvak10}, 
%dynamic slicing~\cite{zhang-icse03},
%zhang-pldi04,
passing/failing traces~\cite{mani-ase10}. Some methods are based on
differencing between passing and failing
runs~\cite{dallmeier-ecoop05}. 
%saha11
Others modify the program state at selected points in the execution of
a failing test, and observe the states' differences. If the failure
still occurs, it will be
reported~\cite{zhang-icse06,cleve-icse05}.  
%jeffrey-issta08,
{\tool} belongs to the class of dynamic approaches. The key different
point in {\tool} is its Bayesian-like rating scheme that needs only a
single test case that causes the crash. Another point is its ability
to map the (invisible) faulty concrete rules back to the original
Makefile.


==> results.tex <==
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{copo_alltrue}
\caption{CoPo .vs \textit{All-true} approach}
\end{figure}


==> results_tb.tex <==
\begin{table}[t]
\centering
\caption{The improvement of {\tool} over the state-of-the-art spectrum-based methods when they are run with  {\tool}}
\label{results_tb}
\begin{tabular}{|l|l|l|l|}
\hline
 						& $EXAM$	& Rank 	& Search space	\\ \hline
Tarantula 				& 37.50 	& 58.25 & 147.17			\\ \hline
{\tool} with Tarantula 	& 5.12 	& 6.23 	& 10.58			\\ \hline
Ochiai 					& 36.54 	& 57.9  	& 147.17			\\ \hline
{\tool} with Ochiai 		& 4.97 	& 6.15 	& 10.58			\\ \hline
\end{tabular}
\end{table}


==> single_bug.tex <==
%\subsection{SPC of single configuration-dependent bug}
 In the case that system contains only bug, all 
configurations in $CF$ are failed by the same bug. Beside property 
\ref{proper_1} and property \ref{proper_2} for the general cases, we 
have the following properties for the fault-causing partial 
configuration $\mathbb{P}$ of the single bug in the system.

\begin{property}
\label{proper_3}
$\mathbb{P}$ is the common subset of all failed configurations, $\mathbb{P} \subseteq \bigcap {c_i}$, where $c_i \in CF$.
\end{property}
%
Indeed, if there exists a failed configuration $c \in CF$, such that $c  
\not \supset \mathbb{P}$, there exists another fault-causing partial 
configuration $\mathbb{P'} \neq \mathbb{P}$ and $c \supset \mathbb{P'}$. 
This leads to that the system contains more than one bug, which 
contradicts with the single bug assumption. For the bug in figure 
\ref{example_bug}, $\mathbb{P} \subseteq c_2 \cap c_7$. 

\subsection{Detail algorithm}

\input{alg_1}

Based on properties \ref{proper_2} and \ref{proper_3},
we propose our method shown in algorithm \ref{alg_1} to detect suspicious partial configuration of a configurable system that containing a single bug, given the test results of the 
system ($CP$ and $CF$). In algorithm \ref{alg_1}, to detect the suspicious partial configuration $partialConfig$, the set of all selections that need to be considered ($consideredSels$) is identified by finding the common subset of all failed configurations in $CF$ (line 3). Next, to construct $partialConfig$, each selections in $consideredSels$ is examined whether it is an element of the suspicious partial configuration or not (line 4 to line 9).
%
For the running example, the detected suspicious partial configuration by algorithm \ref{alg_1} is \{\texttt{PPC\_16K\_PAGES=F}, \texttt{SLAB=T}, \texttt{PPC\_256K\_PAGES=T}, \texttt{LOCKDEP=T}, \texttt{\!SLOB=T}\}.



==> sufficient_necessary.tex <==
%SON
\textbf{SON...}
We aim to detect the suspicious partial configuration (SPC) that causes the configuration-dependent bug in the system. 

\textbf{Assumption}: Every configuration that contains the bug behaves as unexpected (fails at least one test).

For a buggy system whose sets of passed and failed configurations are $CP$ and $CF$ respectively, $SPC$ of the bug is a set of feature selections that must also satisfy both necessity and sufficiency conditions:
\begin{itemize}
\item \textbf{Necessity}: $\forall SPC', SPC' \subsetneq SPC$, such that $\exists c \in CP$, $c \supset SPC'$. 

Because if there exists a passed configuration that contains all $SPC'$, $SPC'$ \textbf{dose not} cause the bug.

\textbf{Corollary}: $SPC$ must satisfy: $\forall c \in \mathbb{C}$, $c \supset SPC \implies c \in CF$, where $\mathbb{C}$ is the configuration space of the system (1).

\item \textbf{Sufficiency}: $\forall SPC', SPC' \supsetneq SPC$, such that $\forall c \in \mathbb{C}$, $c \supset SPC' \implies c \in CF$. 

Indeed, assuming that there exists another \textbf{necessary} $SPC'$, $SPC' \supsetneq SPC$. We have $\forall PC \subsetneq SPC'$, $\exists c \in CP$, $c \supset PC$, which leads to $\exists c \in CP$, $c \supset SPC$, and contradicts with (1). Therefore, $SPC$ must satisfy the sufficiency condition.

\end{itemize}

==> suspicious_stm_detection.tex <==
\section{Suspicious Statement Detection}
\label{statement_detection_section}

For a configuration-dependent bug visible by a $SPC$, not only the statements that implement the interactions of the features in the $SPC$ are likely to be buggy, the executed statements in the failing configurations that are impacted by or have dependency impact on them could be suspicious as well ({\bf O3} and {\bf O4}).
%considered to be suspicious.
%

Given a $SPC$ of a particular bug, let $ES$ be the set of the statements
that implement the interactions between the enabled features ($f_E$s)
in $SPC$; $DS$ be the set of statements that implement the
interactions of $f_E$s with the disabled features ($f_D$s) in $SPC$.
%
In case that there is no $f_D$ ($DS=\emptyset$), if a statement $smt$
has impact on any statement in $ES$, it is considered as
suspicious. However, in the case that $DS \neq \emptyset$, $smt$ is
considered to be faulty only if $smt$ also has dependency impact on at
least one statement in $DS$. Indeed, because if $smt$ has no
dependency impact on any interaction between $f_E$s and $f_D$s, the
impact of $smt$ is not hidden by any $f_D$ when the features in $f_D$s
are enabled ({\bf O3}).

For the running example, the statements that implement the
interactions of \texttt{SLAB}, \texttt{PPC\_256K\_PAGES},
\texttt{LOCKDEP}, and \texttt{\!SLOB} whose enabling make the bug
visible ($ES$) are the statements at lines 4, 11--12, 16, 22, and
24. These statements are also executed in $c_7$, a failing
configuration, and obviously have impact on the interaction between
features in $ES$.
%
Additionally, another statement that has impact on the interaction is
line 1, and it is also suspicious. However, only the statements at
line 1, 11--12, and 22 have impact on the interactions between
\texttt{PPC\_16K\_PAGES} and the features in $ES$. As a result, for
the bug shown in Fig.~\ref{example_bug}, they are the only suspicious
statements.

\textbf{Suspicious statements ranking.} To rank these suspicious
statements, we analyze the execution information in the testing phase
to assign a suspiciousness score to each of these statements. This
could be realized using spectrum-based
techniques~\cite{wong2009survey}. In {\tool}, we use a spectrum-based
tool to access the suspiciousness for only the set of detected
suspicious statements, rather than using them for all executed
statements. Take Tarantula~\cite{tarantula} as an example, the
suspiciousness score of a suspicious statement $stm$:
$$
Suspiciousness(stm) = \frac{N_{CF}/N_F}{N_{CF}/N_F+N_{CS}/N_S}
$$
where:
\begin{itemize}
\item $N_F$ total number of failed test cases
\item $N_S$ total number of successful test cases
\item $N_{CF}$ number of failed test cases that cover $stm$
\item $N_{CS}$ number of successful test cases that cover $stm$
\end{itemize}

\input{alg_3}

\textbf{Describe algorithm 3...}

==> suspiciousness_prop.tex <==
%\subsection{Suspiciousness propagation}
In this phase, given the set of detected statements ($\mathbb{S}$) that implement the interaction between features whose selection is in $\mathbb{P}$, we will analyze the execution traces of during the configurations in $CF$ failing the tests to detect the suspicious statements that are the executed statements having dependency impact on $\mathbb{S}$.

\begin{figure}[h]
\begin{center}
\lstinputlisting[captionpos=b]{executed_stms.c}
\caption{The executed trace of statements in $c_7$}
\label{execution_trace}
\end{center}
\end{figure}

For the set of detected statements that implement the interaction between features whose selection is in $\mathbb{P}$ contains the statements that implement the features that are disabled in $\mathbb{P}$.
